Correspondence between Row-Column Determinants and Quasideterminants of Matrices over Quaternion Algebra

In this paper, we considered the theory of quasideterminants and row and column determinants. We considered the application of this theory to the solving of a system of linear equations in quaternion algebra. We established correspondence between row and column determinants and quasideterminants of matrix over quaternion algebra.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов, Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин,
Элементы теории функций и функционального анализа,
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Mappings of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010)
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008)
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:q-alg/1004.3007} (2010)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М. Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fihtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-rcd форма
   {$1$-\rcd форма}%
   {1-rcd form, vector spaces}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%3%A%a b-CR квазидетерминант
   {$(^a_b)$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index%668%A%A CRcirc- базис модуля
   {$A\CRcirc$\Hyph базис модуля}%
   {A CRcirc basis, module over algebra}%
\Index%667%A%A CRcirc- линейно ависимое множество векторов
   {$A\CRcirc$\Hyph линейно зависимое множество векторов}%
   {CRcirc linearly dependent, Astar module over algebra}%
\Index%666%A%A CRcirc- линейно независимое множество векторов
   {$A\CRcirc$\Hyph линейно независимое множество векторов}%
   {CRcirc linearly independent, Astar module over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%693%A%A линейное отображение модулей
   {$A$\Hyph линейное отображение модулей}%
   {A linear map of modules}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) mapping}%
\Index%680%A%Acr линейное отображение модулей
   {\Acr линейное отображение модулей}%
   {Acr linear map of modules}%
\Index%581%A%Arc  линейно зависимые векторы
   {$A\RCstar$\Hyph  линейно зависимые векторы}%
   {linearly dependent, A vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%580%A%Arc линейно независимые векторы
   {$A\RCstar$\Hyph линейно независимые векторы}%
   {linearly independent, A vector space}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%583%A%Astar линейное отображение векторных пространств
   {$A\star$\Hyph линейное отображение векторных пространств}%
   {Astar linear map of vector spaces}%
\Index%660%A%Astar- модуль
   {$A\star$\Hyph модуль}%
   {Astar-module}%
\Index%665%A%Astar- произведение вектора на скаляр
   {$A\star$\Hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, Astar module}%
\Index%579%A%Astar-произведение вектора на скаляр
   {$A\star$\hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, vector space}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%13%C%crd производная Гато отображения \Vector f D-векторного пространства \Vector V в D-векторное пространство \Vector W
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\Index%649%C%стандартная компонента полилинейного отображения в ассоциативную алгебру
   {стандартная компонента полилинейного отображения в ассоциативную алгебру}%
   {standard component of polylinear map, associative algebra}%
\SetIndexSpace%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%20%D%Drc  линейно зависимые векторные поля
   {\Drc  линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%16%D%drc базис векторного пространства r строк
   {\drc базис векторного пространства \subs строк}%
   {drc basis, r rows vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%19%D%drc векторное пространство r строк
   {\drc векторное пространство \subs строк}%
   {subs rows drc vector space}%
\Index%30%D%drc вектор-функция
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index%33%D%Drc линейно независимые векторные поля
   {\Drc линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%70%D%drc представление группы
   {\drc представление группы}%
   {drc linear representation of group}%
\Index%38%D%drc производная Гато отображения \Vector f D- векторного пространства \Vector V в D- векторное пространство \Vector W
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Index%734%D%Dstar аффинное пространство
   {$D\star$\Hyph аффинное пространство}%
   {Dstar affine space}%
\Index%659%D%Dstar- базис модуля
   {$D\star$\Hyph базис модуля}%
   {D basis, module}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%42%D%Dstar компонента координат вектора \Vector r
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Index%658%D%Dstar линейно зависимые векторы Dstar модуля
   {$D\star$\Hyph линейно зависимые векторы $D\star$\Hyph модуля}%
   {Dstar linearly dependent, module}%
\Index%657%D%Dstar линейно независимые векторы Dstar модуля
   {$D\star$\Hyph линейно независимые векторы $D\star$\Hyph модуля}%
   {Dstar linearly independent, module}%
\Index%71%D%Dstar- модуль
   {$D\star$\Hyph модуль}%
   {Dstar-module}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%40%D%Dstar-векторное пространство
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%44%D%Dstar-произведение вектора на скаляр
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\Index%25%D%rcd базис в векторном пространстве c строк
   {\rcd базис в векторном пространстве \sups строк}%
   {rcd basis, c rows vector space}%
\Index%32%D%rcd линейная оболочка в векторном пространстве
   {\rcd линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%726%N%n алгебра над кольцом
   {$n$\Hyph алгебра над кольцом}%
   {n algebra over ring}%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%49%R%drc базис, дуальный rcd базису в векторном пространстве
   {\drc базис, дуальный \rcd базису в векторном пространстве}%
   {basis dual to basis, rcd vector space}%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главный минор
   {\RC главный минор}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%677%R%RCcirc A- базис модуля
   {$\RCcirc A$\Hyph базис модуля}%
   {RCcirc A basis, module over algebra}%
\Index%676%R%RCcirc A- линейно ависимое множество векторов
   {$\RCcirc A$\Hyph линейно зависимое множество векторов}%
   {RCcirc linearly dependent, starA module over algebra}%
\Index%675%R%RCcirc A- линейно независимое множество векторов
   {$\RCcirc A$\Hyph линейно независимое множество векторов}%
   {RCcirc linearly independent, starA module over algebra}%
\Index%600%R%RCcirc вырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph вырожденная матрица $\mathcal A(A)$\Hyph отображений}%
   {RCcirc singular matrix of A(A) mappings}%
\Index%599%R%RCcirc вырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph вырожденная матрица эндоморфизмов}%
   {RCcirc singular matrix of endomorphisms}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph невырожденная матрица $A(A)$\Hyph отображений}%
   {RCcirc nonsingular matrix of A(A) mappings}%
\Index%598%R%RCcirc невырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph невырожденная матрица эндоморфизмов}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%21%R%rcd  линейно зависимые векторы
   {\rcd  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index%22%R%rcd автоморфизм векторного пространства
   {\rcd автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%758%R%rcd аффинное преобразование
   {\rcd аффинное преобразование}%
   {rcd affine transformation}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%111%R%rcd аффинный базис
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Index%24%R%rcd базис в векторном пространстве
   {\rcd базис в векторном пространстве}%
   {rcd basis, vector space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%29%R%rcd векторное пространство c строк
   {\rcd векторное пространство \sups строк}%
   {sups rows rcd vector space}%
\Index%31%R%rcd изоморфизм векторных пространств
   {\rcd изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%34%R%rcd линейно независимые векторы
   {\rcd линейно независимые векторы}%
   {linearly independent, vector space}%
\Index%35%R%rcd линейное отображение векторных пространств
   {\rcd линейное отображение векторных пространств}%
   {rcd linear map of vector spaces}%
\Index%37%R%rcd линейным Tstar- представление группы
   {\rcd линейным \Ts представление группы}%
   {rcd linear Tstar representation of group}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index%77%S%Dstar- произведением rcd линейного отображения A на скаляр
   {$D\star$\Hyph произведением \rcd линейного отображения $A$ на скаляр}%
   {Dstar product of rcd linear map over scalar}%
\Index%73%S%RCstarS,RCstarT- линейное отображение векторных пространств
   {$(\RCstar S,\RCstar T)$\Hyph линейное отображение векторных пространств}%
   {rcs rct linear map of vector spaces}%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%586%S%star A- product of Astar linear map over scalar
   {$\star A$\Hyph произведением $A\star$\Hyph линейного отображения на скаляр}%
   {starA product of Astar linear map over scalar}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%683%S%star A- произведение Acr линейного отображения на скаляр
   {$\star A$\Hyph произведение \Acr линейного отображения на скаляр}%
   {starA product of Acr linear map over scalar}%
\Index%78%S%star D-векторное пространство
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%674%S%starA- произведение вектора на скаляр
   {$\star A$\Hyph произведение вектора на скаляр}%
   {starA product of vector over scalar, starA module}%
\Index%735%S%starD аффинное пространство
   {$\star D$\Hyph аффинное пространство}%
   {starD affine space}%
\Index%75%S%starD компонента координат вектора \Vector r
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%82%S%starT- представление Omega1 алгебры A в Omega2 алгебре M
   {\sT представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {starT representation of algebra}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%85%S%starT- преобразование
   {\sT преобразование}%
   {starT transformation}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%80%S%starT- сдвиг
   {\sT сдвиг}%
   {starT shift}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%87%T%Tstar- векторное пространство матриц
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index%88%T%Tstar- линейная комбинация векторов
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index%90%T%Tstar- представление Omega1 алгебры A в Omega2 алгебре M
   {\Ts представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {Tstar representation of algebra}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%92%T%Tstar- преобразование
   {\Ts преобразование}%
   {Tstar transformation}%
\Index%93%T%Tstar- преобразование расслоения
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\Index%89%T%Tstar- сдвиг
   {\Ts сдвиг}%
   {Tstar shift}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%99%А%активное starT- представление
   {активное \sT представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%569%А%активное представление группы в многообразии базисов представления
   {активное представление группы $G(f)$ в многообразии базисов представления}%
   {active representation in basis manifold}%
\Index%715%А%активное преобразование многообразия базисов башни представлений
   {активное преобразование многообразия базисов башни представлений}%
   {active transformation of basis, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%106%А%антигомоморфизм расслоенных групп
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%616%А%ассоциатор R алгебры
   {ассоциатор $R$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%689%Б%базис A- модуля
   {базис $A$\Hyph модуля}%
   {basis of A module}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%117%Б%базовый вектор представления группы Ли
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index%123%В%вектор Килинга второго рода
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index%727%В%векторное пространство над полем
   {векторное пространство над полем}%
   {vector space over field}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%130%В%вырожденное линейное отображение D- векторного пространства
   {вырожденное линейное отображение $D$\Hyph векторного пространства}%
   {singular linear map, D vector space}%
\Index%131%В%вырожденное линейное отображение тела
   {вырожденное линейное отображение тела}%
   {singular linear map, division ring}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%698%Г%геометрический объект в координатном представлении, определённом в Omega_2- алгебре
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H, representation g}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%700%Г%геометрический объект, определённый в Omega_2- алгбре
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%156%Д%дифференциал Гато второго порядка отображения \Vector f
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Index%155%Д%дифференциал Гато второго порядка отображения f
   {дифференциал Гато второго порядка отображения $f$}%
   {Gateaux differential of Second Order, division ring}%
\Index%632%Д%дифференциал Гато второго порядка отображения f алгебры
   {дифференциал Гато второго порядка отображения $f$ алгебры}%
   {Gateaux differential of Second Order, algebra}%
\Index%157%Д%дифференциал Гато отображения \Vector f нормированного D- векторного пространства V в нормированное D- векторное пространство W
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Index%158%Д%дифференциал Гато отображения f
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Index%628%Д%дифференциал Гато отображения алгебры
   {дифференциал Гато отображения $f$ алгебры}%
   {Gateaux differential of map, algebra}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\SetIndexSpace%
\Index%576%З%закон ассоциативности для Astar- векторного пространства
   {закон ассоциативности для $A\star$\Hyph векторного пространства}%
   {associative law, Astar vector space}%
\Index%585%З%закон ассоциативности для Astar линейных отображений векторных пространств
   {закон ассоциативности для $A\star$\Hyph линейных отображений векторных пространств}%
   {associative law for Astar linear mappings of vector spaces}%
\Index%662%З%закон ассоциативности для Astar- модуля
   {закон ассоциативности для $A\star$\Hyph модуля}%
   {associative law, Astar module over algebra}%
\Index%162%З%закон ассоциативности для Drc линейных отображений векторных расслоений
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index%163%З%закон ассоциативности для Dstar- векторного пространства
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index%164%З%закон ассоциативности для Dstar- векторных полей
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index%654%З%закон ассоциативности для Dstar- модуля
   {закон ассоциативности для $D\star$\Hyph модуля}%
   {associative law, Dstar module}%
\Index%161%З%закон ассоциативности для rcd линейных отображений векторных пространств
   {закон ассоциативности для \rcd линейных отображений векторных пространств}%
   {associative law for rcd linear maps of vector spaces}%
\Index%671%З%закон ассоциативности для starA- модуля
   {закон ассоциативности для $\star A$\Hyph модуля}%
   {associative law, starA module over algebra}%
\Index%165%З%закон ассоциативности для ковариантного starT- представления
   {закон ассоциативности для ковариантного \sT представления}%
   {associative law for covariant starT representation}%
\Index%166%З%закон ассоциативности для ковариантного Tstar- представления
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for covariant Tstar representation}%
\Index%167%З%закон ассоциативности для парных представлений
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index%168%З%закон ассоциативности произведения расслоенных соответствий
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index%577%З%закон дистрибутивности для Astar- векторного пространства
   {закон дистрибутивности для $A\star$\Hyph векторного пространства}%
   {distributive law, Astar vector space}%
\Index%663%З%закон дистрибутивности для Astar- модуля
   {закон дистрибутивности для $A\star$\Hyph модуля}%
   {distributive law, Astar module over algebra}%
\Index%169%З%закон дистрибутивности для Dstar- векторного пространства
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index%170%З%закон дистрибутивности для Dstar- векторных полей
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index%655%З%закон дистрибутивности для Dstar- модуля
   {закон дистрибутивности для $D\star$\Hyph модуля}%
   {distributive law, Dstar module}%
\Index%672%З%закон дистрибутивности для starA- модуля
   {закон дистрибутивности для $\star A$\Hyph модуля}%
   {distributive law, starA module over algebra}%
\Index%578%З%закон унитарности для Astar- векторного пространства
   {закон унитарности для $A\star$\Hyph векторного пространства}%
   {unitarity law, Astar vector space}%
\Index%664%З%закон унитарности для Astar- модуля
   {закон унитарности для $A\star$\Hyph модуля}%
   {unitarity law, Astar module over algebra}%
\Index%171%З%закон унитарности для Dstar- векторного пространства
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index%172%З%закон унитарности для Dstar- векторных полей
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\Index%656%З%закон унитарности для Dstar- модуля
   {закон унитарности для $D\star$\Hyph модуля}%
   {unitarity law, Dstar module}%
\Index%673%З%закон унитарности для starA- модуля
   {закон унитарности для $\star A$\Hyph модуля}%
   {unitarity law, starA module over algebra}%
\SetIndexSpace%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%176%К%категория Tstar- представлений Omega1 алгебры A
   {категория \Ts представлений $\Omega$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Index%177%К%категория Tstar- представлений Omega1 алгебры из категории A
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of mappings}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%741%К%кватернионная алгебра
   {кватернионная алгебра}%
   {quaternion algebra}%
\Index%184%К%ковариантное starT- представление группы
   {ковариантное \sT представление группы}%
   {covariant starT representation of group}%
\Index%185%К%ковариантное starT- представление расслоенной группы
   {ковариантное \sT представление расслоенной группы}%
   {covariant starT representation of fibered group}%
\Index%186%К%ковариантное Tstar- представление группы
   {ковариантное \Ts представление группы}%
   {covariant Tstar representation of group}%
\Index%187%К%ковариантное Tstar- представление расслоенной группы
   {ковариантное \Ts представление расслоенной группы}%
   {covariant Tstar representation of fibered group}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%614%К%коммутатор R алгебры
   {коммутатор $R$\Hyph алгебры}%
   {commutator of algebra}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%192%К%компонента линейного отображения D- векторного пространчства
   {компонента линейного отображения $D$\Hyph векторного пространчства}%
   {component of linear map, D vector space}%
\Index%193%К%компонента линейного отображения f тела
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Index%194%К%компонента полилинейного отображения \Vector A
   {компонента полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Index%647%К%компонента полилинейного отображения ассоциативной алгебры
   {компонента полилинейного отображения ассоциативной алгебры}%
   {component of polylinear map, associative algebra}%
\Index%195%К%компонента полилинейного отображения тела
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Index%196%К%компонента производной Гато второго порядка отображения \Vector f(\Vector x)
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Index%633%К%компонента производной Гато второго порядка отображения f(x) алгебры
   {компонента производной Гато второго порядка отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of Second Order, algebra}%
\Index%197%К%компонента производной Гато второго порядка отображения тела
   {компонента производной Гато второго порядка отображения тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Index%199%К%компонента производной Гато отображения \Vector f(\Vector x)
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Index%198%К%компонента производной Гато отображения f(x)
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Index%629%К%компонента производной Гато отображения f(x) алгебры
   {компонента производной Гато отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of map, algebra}%
\Index%202%К%контравариантное starT- представление группы
   {контравариантное \sT представление группы}%
   {contravariant starT representation of group}%
\Index%200%К%контравариантное starT- представление расслоенной группы
   {контравариантное \sT представление расслоенной группы}%
   {contravariant starT representation of fibered group}%
\Index%201%К%контравариантное Tstar- представление группы
   {контравариантное \Ts представление группы}%
   {contravariant Tstar representation of group}%
\Index%203%К%контравариантное Tstar- представление расслоенной группы
   {контравариантное \Ts представление расслоенной группы}%
   {contravariant Tstar representation of fibered group}%
\Index%204%К%координатная матрица вектора в rcd базисе
   {координатная матрица вектора в \rcd базисе}%
   {coordinate matrix of vector in rcd basis}%
\Index%691%К%координатная матрица вектора в базисе
   {координатная матрица вектора в базисе}%
   {coordinate matrix of vector in basis, module}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов в векторном пространстве dcr строк
   {координатная матрица множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\Index%207%К%координатная матрица множества векторов в векторном пространстве rcd строк
   {координатная матрица множества векторов в векторном пространстве \rcd строк}%
   {coordinate matrix of set of vectors, rcd vector space}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%697%К%координатное представление в Omega_2- алгебре
   {координатное представление в $\Omega_2$\Hyph алгебре}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%214%К%координатный rcd изоморфизм
   {координатный \rcd изоморфизм}%
   {coordinate rcd isomorphism}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора в rcd базисе
   {координаты вектора в \rcd базисе}%
   {coordinates of vector in rcd basis}%
\Index%692%К%координаты вектора в базисе
   {координаты вектора в базисе}%
   {coordinates of vector in basis, module}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%701%К%координаты геометрического объекта в Omega_2- алгбре
   {координаты геометрического объекта в $\Omega_2$\Hyph алгбре $M$}%
   {coordinates of geometric object, representation g}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%699%К%координаты геометрического объекта в координатном пространстве представления
   {координаты геометрического объекта в координатном пространстве представления}%
   {coordinates of geometric object, coordinate representation}%
\Index%723%К%координаты геометрического объекта в кортеже Omega- алгебр
   {координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinates of geometric object, tower of representations g}%
\Index%222%К%координаты множества векторов в dcr векторном пространстве
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index%223%К%координаты множества векторов в rcd векторном пространстве
   {координаты множества векторов в \rcd векторном пространстве}%
   {coordinates of set of vectors, rcd vector space}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%737%К%координаты точки rcd аффинного пространства относительно базиса
   {координаты точки \rcd аффинного пространства относительно базиса}%
   {coordinates in rcd affine space}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%558%К%координаты элемента представления относительно множества
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%651%К%косо симметричное полилинейное отображение в ассоциативную алгебру
   {косо симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map skew symmetric, associative algebra}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%230%Л%левостороннее ковариантное представление группы
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation of group}%
\Index%231%Л%левостороннее контравариантное представление группы
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation of group}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%237%Л%левый модуль нaд кольцом
   {левый модуль нaд кольцом $D$}%
   {left module over ring}%
\Index%661%Л%левый модуль над D- алгеброй A
   {левый модуль над $D$\Hyph алгеброй $A$}%
   {left module over algebra}%
\Index%731%Л%левый сдвиг R- модуля
   {левый сдвиг $R$\Hyph модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index%686%Л%линейная комбинация векторов A- модуля
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Index%98%Л%линейнное отображение тела, порождённое отображением G
   {линейное отображение тела, порождённое отображением $G$}%
   {linear map generated by map, division ring}%
\Index%688%Л%линейно зависимое множество A- модуля
   {линейно зависимое множество $A$\Hyph модуля}%
   {linear dependent vectors, module}%
\Index%687%Л%линейно независимое множество A- модуля
   {линейно независимое множество $A$\Hyph модуля}%
   {linear independent vectors, module}%
\Index%608%Л%линейное отображение  R_1 модуля в R_2 модуль
   {линейное отображение  $R_1$\Hyph модуля $A_1$ в $R_2$\Hyph модуль $A_2$}%
   {linear mapping of R_1 module into R_2 module}%
\Index%242%Л%линейное отображение D- векторных пространств над полем F
   {линейное отображение $D$\Hyph векторных пространств над полем $F$}%
   {linear map over field, vector space}%
\Index%610%Л%линейное отображение R алгебры в R алгебру
   {линейное отображение $R$\Hyph алгебры $A_1$ в $R$\Hyph алгебру $A_2$}%
   {linear mapping of R algebras}%
\Index%613%Л%линейное отображение R модуля в R модуль
   {линейное отображение $R$\Hyph модуля $A_1$ в $R$\Hyph модуль $A_2$}%
   {linear mapping of R modules}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear mapping of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%740%Л%линейное преобразование rcd аффинного пространства
   {линейное преобразование \rcd аффинного пространства}%
   {linear transformation, rcd affine space}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%681%М%матрица Acr линейного отображения модуля
   {матрица \Acr линейного отображения модуля}%
   {matrix of Acr linear map}%
\Index%584%М%матрица Astar линейного отображения
   {матрица $A\star$\Hyph линейного отображения}%
   {matrix of Astar linear map}%
\Index%251%М%матрица rcd линейного отображения
   {матрица \rcd линейного отображения}%
   {matrix of rcd linear map}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear mappings}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of mappings}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения D- векторного пространства
   {матрица Якоби\Hyph Гато отображения $D$\Hyph векторного пространства}%
   {Jacobi Gateaux matrix of map, D vector space}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие базисов \rcd аффинного пространства
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни Tstar- представлений в башню Tstar- представлений
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index%738%Н%начало системы координат star D аффинного пространства
   {начало системы координат $\star D$\Hyph аффинного пространства}%
   {origin of coordinate system of starD affine space}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor, algebra}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%313%Н%непрерывная функция над алгебро1
   {непрерывная функция над $D$\Hyph алгебро1}%
   {continuous function, algebra}%
\Index%280%Н%непрерывная функция тела
   {непрерывная функция тела}%
   {continuous function, division ring}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%346%Н%норма на D- алгебре
   {норма на $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%285%Н%норма отображения  тела
   {норма отображения  тела}%
   {norm of map, division ring}%
\Index%286%Н%норма отображения \Vector A нормированного D-векторного пространства
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Index%314%Н%норма отображения в D- алгебру
   {норма отображения в $D$\Hyph алгебру}%
   {norm of map, algebra}%
\Index%343%Н%нормированная D- алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%287%Н%нормированное D- векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\SetIndexSpace%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map, division ring}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%304%О%орбита Tstar- представления группы
   {орбита \Ts представления группы}%
   {orbit of Tstar  representation of group}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормальный базис
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормальный базис
   {ортонормальный базис}%
   {Orthonornal Basis, division ring}%
\Index%638%О%ортонормированый базис в пространстве Минковского
   {ортонормированый базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг rcd аффинного пространства
   {параллельный сдвиг \rcd аффинного пространства}%
   {parallel shift, rcd affine space}%
\Index%684%П%парные представления D- алгебры
   {парные представления $D$\Hyph алгебры}%
   {twin representations of D algebra}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное starT- представление
   {пассивное \sT представление}%
   {passive starT representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%695%П%пассивное представление группы в многообразии базисов представления
   {пассивное представление группы $G(f)$ в многообразии базисов представления}%
   {passive representation in basis manifold}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric, division ring}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%342%П%полилинейное отображение (n)-D-векторных пространств
   {полилинейное отображение $(n)$\hyph $D$\hyph векторных пространств}%
   {polylinear map of D vector spaces}%
\Index%609%П%полилинейное отображение алгебр
   {полилинейное отображение алгебр}%
   {polylinear map of algebras}%
\Index%621%П%полилинейное отображение модулей
   {полилинейное отображение модулей}%
   {polylinear map of modules}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric, division ring}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%351%П%последовательность Коши в нормированное теле
   {последовательность Коши в нормированное теле}%
   {Cauchy sequence, valued division ring}%
\Index%271%П%последовательность Коши в нормированном алгебре
   {последовательность Коши в нормированном алгебрае}%
   {Cauchy sequence, normed algebra}%
\Index%241%П%последовательность Коши в нормированном кольце
   {последовательность Коши в нормированном кольце}%
   {Cauchy sequence, normed ring}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%355%П%правостороннее ковариантное представление группы
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation of group}%
\Index%356%П%правостороннее контравариантное представление группы
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation of group}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%361%П%правый модуль нaд кольцом
   {правый модуль нaд кольцом $D$}%
   {right module over ring}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%460%П%предел последовательности в нормированной алгебре
   {предел последовательности в нормированной алгебре}%
   {limit of sequence, normed algebra}%
\Index%467%П%предел последовательности в нормированном кольце
   {предел последовательности в нормированном кольце}%
   {limit of sequence, normed ring}%
\Index%364%П%предел последовательности в нормированном теле
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%703%П%представитель геометрического объекта в Omega_2- алгбре
   {представитель геометрического объекта в $\Omega_2$\Hyph алгбре}%
   {representative of geometric object, representation g}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%384%П%принцип инвариантности в представлении универсальной алгебры
   {принцип инвариантности в представлении универсальной алгебры}%
   {invariance principle, representation g}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%390%П%произведение групп
   {произведение групп}%
   {product of groups}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка отображения f
   {производная Гато второго порядка отображения $f$}%
   {Gateaux derivative of Second Order, division ring}%
\Index%626%П%производная Гато второго порядка отображения алгебры
   {производная Гато второго порядка отображения алгебры}%
   {Gateaux derivative of Second Order, algebra}%
\Index%397%П%производная Гато отображения f
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Index%398%П%производная Гато отображения Vector f нормированого D- векторного пространства Vector V в нормированное D- векторное пространство Vector W
   {производная Гато отображения $\Vector f$ нормированого $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Index%627%П%производная Гато отображения алгебры
   {производная Гато отображения алгебры}%
   {Gateaux derivative of map, algebra}%
\Index%399%П%производная Гато порядка n отображения \Vector f
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Index%634%П%производная Гато порядка n отображения f алгебры
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, algebra}%
\Index%400%П%производная Гато порядка n отображения f тела
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит Tstar- представления
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%412%П%прямое произведение Tstar- представлений группы
   {прямое произведение \Ts представлений группы}%
   {direct product of Tstar representations of group}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%441%С%свободное Tstar- представление группы
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато отображения f^j по переменным v^i, v^j
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%456%С%стандартная F- компонента линейного отображения f
   {стандартная $F$\Hyph компонента линейного отображения $f$}%
   {standard component of linear map, division ring}%
\Index%458%С%стандартная компонента дифференциала Гато отображения f
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Index%459%С%стандартная компонента квадратичного отображения f над полем F
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения f тела
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Index%630%С%стандартная компонента производной Гато отображения f
   {стандартная компонента производной Гато отображения $f$}%
   {standard component of Gateaux derivative, algebra}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%
\Index%574%С%стандартная компонента тензора в тензорном произведении алгебр
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Index%464%С%стандартное F- представление линейного отображения тела
   {стандартное $F$\Hyph представление линейного отображения тела}%
   {linear map, standard representation, division ring}%
\Index%465%С%стандартное представление дифференциала Гато отображения тела над полем F
   {стандартное представление дифференциала Гато отображения тела над полем $F$}%
   {Gateaux differential, standard representation, division ring}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%648%С%стандартное представление полилинейного отображения в ассоциативную алгебру
   {стандартное представление полилинейного отображения в ассоциативную алгебру}%
   {polylinear map, standard representation, associative algebra}%
\Index%470%С%стандартное представление полилинейного отображения тела
   {стандартное представление полилинейного отображения тела}%
   {polylinear map, standard representation, division ring}%
\Index%631%С%стандартное представление производной Гато отображения над алгеброй
   {стандартное представление производной Гато отображения над алгеброй}%
   {Gateaux derivative, standard representation, algebra}%
\Index%471%С%стандартные координаты rcd базиса
   {стандартные координаты \rcd базиса}%
   {standard coordinates of rcd basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%618%С%структурные константы алгебры над кольцом
   {структурные константы алгебры $P$ над кольцом $D$}%
   {structural constants of algebra}%
\Index%473%С%структурные константы тела D над полем F
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%682%С%сумма Acr линейных отображений модуля
   {сумма \Acr линейных отображений модуля}%
   {sum of Acr linear maps, module}%
\Index%475%С%сумма rcd линейных отображений
   {сумма \rcd линейных отображений}%
   {sum of rcd linear maps, rcd vector spaces}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%323%С%суперпозиция координат эндоморфизма представления и элемента
   {суперпозиция координат эндоморфизма представления $f$ и элемента $m$}%
   {superposition of coordinates, representation}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%652%Т%тензорная степень алгебры $A$
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Index%480%Т%тензорное произведение D- векторных пространств
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index%481%Т%тензорное произведение Dstar векторных пространств
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index%573%Т%тензорное произведение алгебр
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Index%482%Т%тензорное произведение колец над коммутативным кольцом
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index%483%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%484%Т%тензорное произведение тел
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%487%Т%топологическое drc векторное пространство
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%493%У%уравнение Килинга
   {уравнение Килинга}%
   {Killing equation}%
\Index%494%У%уравнение Килинга второго рода
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%500%Ф%фундаментальная последовательность в нормированное теле
   {фундаментальная последовательность в нормированное теле}%
   {fundamental sequence, valued division ring}%
\Index%243%Ф%фундаментальная последовательность в нормированном алгебре
   {фундаментальная последовательность в нормированном алгебре}%
   {fundamental sequence, normed algebra}%
\Index%642%Ф%фундаментальная последовательность в нормированном кольце
   {фундаментальная последовательность в нормированном кольце}%
   {fundamental sequence, normed ring}%
\Index%502%Ф%функция \gi n D- значных переменных
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index%501%Ф%функция D- векторного пространства V в D- векторное пространство W, дифференцируемая по Гато
   {функция $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector W$, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, D vector space}%
\Index%625%Ф%функция алгебры, дифференцируемая по Гато
   {функция алгебры, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, algebra}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%505%Ф%функция тела, дифференцируемая по Гато
   {функция тела, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, division ring}%
\Index%506%Ф%функция, непрерывная по совокупности аргументов
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $R$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%510%Ч%частная crd производная Гато отображения fb по переменной xa
   {частная \crd производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial crd derivative of map with respect to variable, D vector space}%
\Index%511%Ч%частная drc производная Гато отображения f^b по переменной x^a
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато отображения f^j по переменной v^i
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Index%513%Ч%частное линейное отображение переменной v^i
   {частное линейное отображение переменной $v^i$}%
   {partial linear map of variable}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%516%Э%эффективное Tstar- представление группы
   {эффективное \Ts представление группы}%
   {effective Tstar representation of group}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%517%Э%эффективное представление Omega- алгебры A
   {эффективное представление $\Omega$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $R$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%522%Я%ядро линейного отображения D- векторного пространства
   {ядро линейного отображения $D$\Hyph векторного пространства}%
   {kernel of linear map, D vector space}%
\Index%523%Я%ядро линейного отображения тела
   {ядро линейного отображения тела}%
   {kernel of linear map, division ring}%
\Index%524%Я%ядро неэффективности Tstar- представления группы G
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of Tstar representation of group}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%

\CloseIndex


==> Preface.Dtmt.Russian.tex <==
%auto-ignore
\input{Preface.Dtmt.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Предисловие}
\fi
\section{Предисловие}

Линейная алгебра является мощным инструментом, которым мы пользуемся в
различных областях математики, включая математический анализ,
аналитическую и дифференциальную геометрии, теорию дифференциальных уравнений,
теорию оптимального управления.
Линейная алгебра накопила богатый набор различных методов.
Так как некоторые методы имеют общий конечный результат,
это даёт нам возможность выбрать наиболее эффективный метод в зависимости
от характера расчётов или выполняемых построений.

При переходе от линейной алгебры над полем к линейной алгебре над
телом мы хотим сохранить как можно больше
инструментария, которым мы регулярно пользуемся. Уже в начале XX
века, вскоре после после создания Гамильтоном алгебры
кватернионов, математики стали искать ответ, как выглядит алгебра
с некоммутативным умножением. В частности возникла проблема
как определить
детерминант матрицы с элементами, принадлежащими некоммутативному кольцу.
Такой детерминант также
называют некоммутативным детерминантом.

Возникло немало подходов к определению некоммутативного детерминанта.
Но  ни один из введённых некоммутативных детерминантов в полной мере не сохранял
те свойства, которыми он обладал для матриц над полем. Более того,
в работе \citeBib{J. Fan: Determinants} доказано, что не существует единого
детерминантного функционала, который бы расширял определение
детерминанта вещественных матриц для матриц над телом
кватернионов. Поэтому поиски решения проблемы определения некоммутативного
детерминанта продолжаются до сих пор.

В данной работе мы
рассматриваем два подхода к определению некоммутативного
детерминанта:  строчно\Hyph столбцовые определители и
квазидетерминанты.

Строчно\Hyph столбцовые определители
являются расширением классического
определения детерминанта, но с заранее определенным порядком
элементов в каждом из слагаемых детерминанта.
При использовании строчно\Hyph столбцовых определителей,
мы получаем решение системы линейных уравнений
над  кватернионной алгеброй согласно правилу Крамера.

Квазидетерминант
появился в результате анализа процесса обращения матрицы.
При использовании квазидетерминанта,
решение системы линейных уравнений
над  кватернионной алгеброй аналогично методу Гаусса.

Общим в определении строчно-столбцовых
определителей и квазидетерминантов является, что в обоих случаях
квадратной матрице $n$-го порядка с некоммутативными элементами
ставится в соответствие не один определитель, а некоторое их
множество ($n^{2}$ квазидетерминантов и соответственно $n$
строчных и $n$ столбцовых определителей).

Квазидетерминанты нашли
в последнее время широкое применение, как в области линейной
алгебры
(\citeBib{Lauve: Quantum coordinates,Suzuki: Noncommutative spectral decomposition}),
так и физики
(\citeBib{Gilson Nimmo Ohta,Haider Hassan,Li Nimmo: Darboux transformations}).
Сравнительно недавно введенные строчно-столбцовые
определители (\citeBib{0702447}) менее известны. Целью данной статьи является
установление соответствия между строчно-столбцовыми
определителями и квазидетерминантами матриц над кватернионной
алгеброй. Авторы полны надежды  что установленное соответствие
может дать обоюдное развитие как теории квазидетерминантов, так и
строчно-столбцовых определителей.

\section{Соглашение об обозначениях}

Существуют различные формы записи элементов матрицы.
В данной статье элемент матрицы $\bfA$ мы обозначать $a_{ij}$.
При этом индекс $i$ нумерует строки, а индекс $j$
нумерует столбцы.

Для обозначения различных миноров
матрицы $\bfA$ мы будем пользоваться следующей записью
\begin{description}
\item
[\ShowEq{row i}\ \ ]
строка с индексом $i$
\item [\ShowEq{A from rows S}\ \ ]
минор, полученный из $A$ выбором строк с индексом
из множества $S$
\item [\ShowEq{A without row i}\ \ ]
минор, полученный из $A$ удалением
строки $\rowA i$
\item [\ShowEq{A without rows S}\ \ ]
минор, полученный из $A$ удалением строк с индексом
из множества $S$
\item [\ShowEq{column j}\ \ ]
столбец с индексом $j$
\item
[\ShowEq{A from columns T}\ \ ]
минор, полученный из $A$ выбором
столбцов с индексом из множества $T$
\item [\ShowEq{A without column j}\ \ ]
минор, полученный из $A$ удалением
столбца $\colA j$
\item [\ShowEq{A without columns T}\ \ ]
минор, полученный из $A$ удалением
столбцов с индексом из множества $T$
\item [\ShowEq{matrix, replacing its column}\ \ ]
матрица, которую получим из матрицы
$\bfA$ заменой ее  $j$-го столбца столбцом  ${\rm {\bf b}}$
\item [\ShowEq{matrix, replacing its row}\ \ ]
матрица, которую получим из матрицы  $\bfA$ заменой ее
$i$-й строки строкой ${\rm {\bf b}}$
\end{description}

Рассмотренные обозначения могут быть скомбинированы. Например, запись
\[
\rowcolAw {ii}{k.}{\rm {\bf b}}
\]
означает замену строки с номером $k$ матрицей ${\rm {\bf b}}$
с последующим удалением строки с номером $i$
и столбца с номером $i$.

Как отмечалось в разделе
\xRef{0701.238}{section: Biring}
мы можем определить два вида произведения матриц:
либо произведение строк первой матрицы на столбцы второй,
либо произведение столбцов первой матрицы на строки второй.
Однако согласно теореме
\xRef{0701.238}{theorem: rcstar transpose}
это произведение симметрично относительно операции транспонирования.
Поэтому в статье мы ограничимся
традиционным произведением строк первой матрицы на столбцы второй,
и мы не будем указывать явно операцию как это было сделано
в \citeBib{0701.238}.

\section{Предварительные замечания}
Теорию определителей матриц с некоммутативными элементами, можно
условно разделить на три группы относительно методов их
определения. Обозначим через ${\rm M}( {n,\bf K})$ кольцо матриц
с элементами из кольца $\bf K$.
Один из способов
определения детерминанта матрицы из
${\rm M}\left( {n,\bf K} \right)$ --- следующий
(\citeBib{H. Aslaksen,N. Cohen S. De Leo,Dyson: Quaternion determinants}).

\begin{definition}
Пусть функционал
\ShowEq{Quaternion determinants}
удовлетворяет следующим аксиомам.
\begin{itemize}
\item []  {\bf Аксиома 1.}
 $\rm{d}\left( {\bfA} \right) = 0$ тогда и только тогда,
  когда $\bfA$ -- вырожденная (необратимая).
\item [] {\bf Аксиома 2.}
\ShowEq{Quaternion determinants, product}
\item [] {\bf Аксиома 3.}
 Если матрица $\bfA'$ получается из матрицы ${\rm {\bf
 A}}$  прибавлением ее произвольной строки умноженной слева с ее
 другой строкой или ее произвольного столбца умноженного справа с ее
 другим столбцом, тогда
\ShowEq{Quaternion determinants, obtain}
\end{itemize}
Тогда значение функционала ${\rm d}$ называется определителем
матрицы $\bfA\in {\rm M}\left( {n,\bf K}
\right)$.
\qed
\end{definition}

 Примерами таких функционалов являются известные определители Дьедонне и Стади.
В \citeBib{H. Aslaksen} доказано, что определители, которые удовлетворяют
аксиомы 1, 2, 3, принимают свое значение в некотором
коммутативном подмножестве кольца.
 Также для них не имеет смысла
  такое свойство обычных определителей как разложение по минорам строки или столбца.
  Поэтому детерминантное представление обратной матрицы с
   помощью только таких определителей невозможно.
    Всё  это является причиной, которая заставляет вводить
 детерминантные функционалы, не удовлетворяющие всем
 вышеприведенным аксиомам. При этом аксиома 1 рассматривается в
 \citeBib{Dyson: Quaternion determinants}
 как необходимая для определения детерминанта.

При другом подходе определитель квадратной матрицы над
некоммутативным кольцом строится
 как  рациональная функция от элементов матрицы.
 Наибольшего успеха здесь достигли И. М. Гельфанд и В. С. Ретах
 своей теорией квазидетерминантов
(\citeBib{Gelfand Retakh 1991,Gelfand Retakh 1992}). Введение в
 теорию квазидетерминантов будет изложено в разделе
\ref{section: quasideterminant}.

При третьем подходе детерминант матрицы с
некоммутативными элементами определяется, как альтернированная
сумма $n!$ произведений элементов матрицы, но с определенным
фиксированным порядком множителей в каждом из них.
 Е. Г. Мур был первый, кто достиг выполнения ключевой аксиомы 1
  при таком определении некоммутативного детерминанта. Мур
  сделал это не для всех квадратных матриц, а только для эрмитовых.
   Он определил детерминант  эрмитовой
   матрицы\footnote{\AddIndex{Эрмитова матрица}{hermitian matrix}
   - это такая матрица $\bfA=(a_{ij})$, что
   $a_{ij}=\overline{a_{ji}}$.}
   $\bfA=(a_{ij})_{n\times n}$
     над телом с инволюцией  индукцией по
$n$  следующим образом (см. \citeBib{Dyson: Quaternion determinants})
\begin{equation}
\EqLabel{determinant, recursive definition, kyr}
  {\rm Mdet  {\bf A}}
  = {\left\{
{{\begin{array}{ll}%{*{20}c}
 a_{11}, &n = 1
\\
 \sum\limits_{j = 1}^n \varepsilon _{ij} a_{ij}
 {\rm Mdet} \left( \bfA
{\rm (}i \to j{\rm )} \right),&n > 1
\end{array}} } \right.}
\end{equation}
Здесь $\varepsilon _{kj} = {\left\{ {{\begin{array}{rl}
 1,&i = j\\
 - 1,&i \ne j
\end{array}} } \right.}$, а через $ {\bfA(i \to j
)}$ обозначена матрица, которая получается из матрицы ${\rm {\bf
A}}$ последовательным применением замены   $j$-го столбца $i$-м и
вычеркивания $i$-ых строки и столбца. Другое определение этого
детерминанта представлено в \citeBib{H. Aslaksen} в терминах подстановок:
\[
{\rm{Mdet}}\, \bfA = {\sum\limits_{\sigma \in S_n}
{{\left| {\sigma} \right|}{a_{n_{11} n_{12}}  \cdot \ldots \cdot
a_{n_{1l_1}  n_{11}}  \cdot }} {a_{n_{21} n_{22}}} \cdot \ldots
\cdot {a_{n_{rl_1}  n_{r1}}}}.
\]
Здесь $S_n $ -- симметрическая группа $n$ элементов.
Разложение подстановки   $\sigma $  в циклы имеет
вид:
\[
\sigma = \left( {n_{11} \ldots n_{1l_1} }  \right)\left( {n_{21}
\ldots n_{2l_{2}} }  \right)\ldots \left( {n_{r1} \ldots
n_{rl_{r}} }  \right).
\]

Однако, не существовало никакого обобщения определения
детерминанта Мура для произвольных квадратных матриц.  Ф. Д.
Дайсон отмечал важность этой задачи в работе
\citeBib{Dyson: Quaternion determinants}.

В статьях
\citeBib{L. Chen: Definition of determinant,L. Chen: Inverse matrix}
Чен
Лонгхуан предложил следующее определение детерминанта квадратной матрицы
над телом кватернионов $\bfA=(a_{ij}) \in {\rm M}\left(
{n,\bf H} \right)$:
\[
\begin{array}{c}
  \det \bfA = {\sum\limits_{\sigma \in S_n}  {\varepsilon
\left( {\sigma}  \right)a_{n_1 i_{2}}  \cdot a_{i_{2} i_{3}}
\ldots \cdot a_{i_{s} n_1}  \cdot} } \ldots \cdot a_{n_{r}
k_{2}}  \cdot \ldots \cdot a_{k_{l} n_{r}}, \\
   \sigma = \left( {n_1 i_{2} \ldots i_{s}}  \right)\ldots \left(
{n_{r} k_{2} \ldots k_{r}}  \right),\\
  n_1 > i_{2} ,i_{3} ,\ldots ,i_{s} ;\ldots ,n_{r} > k_{2} ,k_{3}
,\ldots ,k_{l}, \\
  n = n_1 > n_{2} > \ldots > n_{r} \ge 1.
\end{array}
\]
Несмотря на то, что такой определитель не удовлетворяет аксиоме 1,
Л. Чен  получил детерминантное  представление обратной матрицы. Но
его определитель также нельзя  разложить
  по минорам строки или столбца (за исключением $n$-й строки).
Поэтому Л. Чен также не получил классическую присоединенную матрицу.
Для $\bfA = \left( {\alpha_1 ,\ldots ,\alpha _{m}}
\right)$ над телом кватернионов  ${\rm {\mathbb{H}}}$, если
${\left\| {\bfA} \right\|}:=\det(\bfA^*{\rm
{\bf A}}) \ne 0$, тогда $\exists \bfA^{ - 1} = \left(
{b_{jk}} \right)$, где
\[
\overline {b_{jk}}  = {\frac{1}{{{\left\| {\bfA}
\right\|}}}}\omega _{kj}, \quad \left( {j,k = 1,2,\ldots ,n}
\right),
\]
\[
\omega _{kj} = \det \left( {\alpha_1 \ldots \alpha _{j - 1}
\alpha _n \alpha _{j + 1} \ldots \alpha _{n - 1} \delta _{k}}
\right)^* \left( {\alpha_1 \ldots \alpha _{j - 1} \alpha
_n \alpha _{j + 1} \ldots \alpha _{n - 1} \alpha _{j}}
\right){\rm .}
\]
\noindent Здесь $\alpha _{i} $ -- $i$-й столбец  $\bfA$,
$\delta _{k} $ --  $n$\Hyph мерный столбец с 1 в $k$-й строке и 0 в
других. Л. Чен определил ${\left\| {\bfA}
\right\|}:=\det(\bfA^*\bfA)$, как двойной
детерминант. Решение правой системы линейных уравнений
\[{\sum\nolimits_{j = 1}^{n} {\alpha _{j} x_{j} = \beta} } \]
 над
${\rm {\mathbb{H}}}$, если ${\left\| {\bfA} \right\|} \ne
0$, представлено следующей формулой, которую автор называет
крамеровской
\[
x_{j} = {\left\| {\bfA} \right\|}^{ - 1}\overline {{\rm
{\bf D}}_{j}}, \,\,\,\forall j=\overline{1,n}
\]
\noindent где
\[
{\rm {\bf D}}_{j} = \det \left( {{\begin{array}{*{20}c}
 {\alpha_1^* }  \hfill \\
 { \vdots}  \hfill \\
 {\alpha _{j - 1}^* }  \hfill \\
 {\alpha _n^* }  \hfill \\
 {\alpha _{j + 1}^* }  \hfill \\
 {\vdots} \hfill \\
 {\alpha _{n - 1}^* }  \hfill \\
 {\beta ^* } \hfill \\
\end{array}} } \right)\left( {{\begin{array}{*{20}c}
 {\alpha_1}  \hfill & {\ldots}  \hfill & {\alpha _{j - 1}}  \hfill &
{\alpha _n}  \hfill & {\alpha _{j + 1}}  \hfill & {\ldots}
\hfill & {\alpha _{n - 1}}  \hfill & {\alpha _{j}}  \hfill \\
\end{array}} } \right).
\]
\noindent Здесь $\alpha _{i} $ -- $i$-й столбец матрицы ${\rm {\bf
A}}$, $\alpha _{i}^*  $ --- $i$-я строка матрицы ${\rm {\bf
A}}^* $, $\beta ^* $ --- $n$\Hyph мерная вектор\Hyph строка
сопряженная с
 $\beta $.

 В данной работе мы рассматриваем теорию строчных и столбцовых
 определителей, которая развивает классический подход к
 определению детерминанта матрицы, но с заранее определенным
 порядком множителей в каждом из слагаемых детерминанта.


==> Qdtmt.Russian.tex <==
%auto-ignore
\input{Qdtmt.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Квазидетерминант}
\fi

\section{Квазидетерминант}
\label{section: quasideterminant}

\begin{theorem}
\label{theorem: inverse matrix}
Предположим, что матрица\footnote{Это утверждение
и его доказательство основаны
на утверждении 1.2.1 из \citeBib{math.QA-0208146}
для матриц над свободным кольцом с делением.}
\ShowEq{matrix nxn}
имеет обратную матрицу $A^{-1}$.
Тогда минор обратной матрицы
удовлетворяет следующему равенству, при условии, что рассматриваемые
обратные матрицы существуют,
\ShowEq{inverse minor, quasideterminant}
\end{theorem}
\begin{proof}
Определение обратной матрицы
приводит к системе линейных уравнений
\ShowEq{inverse minor, quasideterminant, 1}
Мы умножим \EqRef{inverse minor, quasideterminant, 1, 1} на
\ShowEq{inverse minor, quasideterminant, 3}
Теперь мы можем подставить
\EqRef{inverse minor, quasideterminant,3} в
\EqRef{inverse minor, quasideterminant, 1, 2}
\ShowEq{inverse minor, quasideterminant, 4}
\EqRef{inverse minor, quasideterminant}
следует из \EqRef{inverse minor, quasideterminant, 4}.
\end{proof}

\begin{corollary}
\label{corollary: inverse matrix, quasideterminant}
Предположим, что матрица $\bfA$
имеет обратную матрицу.
Тогда элементы обратной матрицы удовлетворяют
равенству
\ShowEq{element of inverse matrix}
\qed
\end{corollary}

\begin{example}
Рассмотрим матрицу
\ShowEq{inverse matrix 2x2, 0}
Согласно \EqRef{element of inverse matrix}
\ShowEq{inverse matrix 2x2}
\qed
\end{example}

Мы называем матрицу
\ShowEq{Hadamard inverse of matrix}
\AddIndex{обращением Адамара матрицы}{Hadamard inverse of matrix}
\footnote{\citeBib{q-alg-9705026}-\href{http://arxiv.org/PS_cache/q-alg/pdf/9705/9705026.pdf\#Page=4}{стр. 4}}
\ShowEq{matrix nxn}

\begin{definition}
\label{definition: quasideterminant}
\AddIndex{$(ji)$\hyph квазидетерминант}
{j i quasideterminant}
матрицы $\bfA$
- это формальное выражение
\ShowEq{j i quasideterminant definition}
Мы можем рассматривать $(ji)$\hyph квазидетерминант
как элемент матрицы
\ShowEq{quasideterminant definition},
которую мы будем называть
\AddIndex{квазидетерминантом}
{quasideterminant definition}.
\qed
\end{definition}

\begin{theorem}
Выражение для
$(ji)$\hyph квазидетерминанта
имеет форму
\ShowEq{quasideterminant, expression}
\end{theorem}
\begin{proof}
Утверждение  следует
из \EqRef{element of inverse matrix} и
\EqRef{j i quasideterminant definition}.
\end{proof}

\begin{theorem}
\label{theorem: inverse matrix, delta}
Пусть
\ShowEq{unit matrix order 2}
Тогда
\ShowEq{inverse matrix, unit}
\end{theorem}
\begin{proof}
Из \EqRef{inverse matrix, 1 1}
и \EqRef{inverse matrix, 2 2} очевидно, что
\ShowEq{inverse matrix, unit 1 1}
и
\ShowEq{inverse matrix, unit 2 2}
Тем не менее выражение для
\ShowEq{inverse matrix, unit 1 2}
и
\ShowEq{inverse matrix, unit 2 1}
не может быть определено из
\EqRef{inverse matrix, 1 2} и \EqRef{inverse matrix, 2 1}
так как
\ShowEq{inverse matrix, unit 01}
Мы можем преобразовать эти выражения. Например
\ShowEq{inverse matrix, unit 02}
Мы непосредственно видим, что
\ShowEq{inverse matrix, unit 03}
Таким же образом мы можем найти, что
\ShowEq{inverse matrix, unit 04}
Это завершает доказательство \EqRef{inverse matrix, unit}.
\end{proof}

Из доказательства теоремы
\ref{theorem: inverse matrix, delta} видно,
что мы не всегда можем пользоваться равенством
\EqRef{element of inverse matrix}
для определения элементов обратной матрицы
и необходимы дополнительные преобразования для решения этой
задачи.
Из теоремы
\xRef{0701.238}{theorem: singular matrix and quasideterminant}
следует, что если
\[
\mathrm{rank}
\matrixNN
\le n-2
\]
то $|\bfA|_{ij}$, $i=1$, ..., $n$, $j=1$, ..., $n$,
не определён.
Из этого следует, что хотя квазидетерминант является мощным
инструментом, возможность пользоваться определителем является
серьёзным преимуществом.

\begin{theorem}
\label{theorem: two products equal}
Если матрица $\bfA$ имеет обратную матрицу, то для любых матриц
${\rm {\bf B}}$ и ${\rm {\bf C}}$ из равенства
\ShowEq{two products equal, 1}
следует равенство
\ShowEq{two products equal, 2}
\end{theorem}
\begin{proof}
Равенство \EqRef{two products equal, 2} следует из
\EqRef{two products equal, 1}, если обе части равенства
\EqRef{two products equal, 1} умножить на $\bfA^{-1}$.
\end{proof}

\begin{theorem}
\label{theorem: nonsingular system of linear equations}
Решение невырожденной системы линейных уравнений
\ShowEq{nonsingular system of linear equations} определено однозначно
и может быть записано в любой из следующих форм\footnote{Смотри аналогичное утверждение
в теореме
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=19}{1.6.1}.
}
\ShowEq{nonsingular system of linear equations, solution}
\end{theorem}
\begin{proof}
Умножая обе части равенства \EqRef{nonsingular system of linear equations}
слева на $\bfA^{-1}$, мы получим
\EqRef{nonsingular system of linear equations, solution, matrix}.
Пользуясь определением
\ref{definition: quasideterminant},
мы получим \EqRef{nonsingular system of linear equations, solution, quasideterminant}.
Решение системы единственно в силу теоремы
\ref{theorem: two products equal}.
\end{proof}



==> RQdtmt.Russian.tex <==
%auto-ignore
\input{RQdtmt.Eq}

%\ifx\PrintBook\undefined
%\else
\Chapter{Соответствие между строчно\hyph столбцовыми определителями и квазидетерминантами}
%\fi

\begin{theorem}
\label{theorem: quasi row column determinant}
Если $\bfA \in {\rm
M}(n,{\rm {\mathbb{H}}})$ - обратимая матрица, то для
произвольных $p,q=1$, ..., $n$ мы имеем следующие представления
квазидетерминанта
\ShowEq{quasi row column determinant}
\def\theDate{September 18}
\ifx\AleksComment\theDate
\begin{equation}\label{kyr12}
  \mid{\rm {\bf A}}\mid_{pq}=\frac{{\rm{ddet}}{ \rm{\bf A}}\cdot \overline{{\rm{cdet}} _{q} ({\rm {\bf A}}^{
* }{\rm {\bf A}})_{.\,q} \left( {{\rm {\bf a}}_{.{\kern 1pt} p}^{
*} } \right)}}{{\rm n}({\rm{cdet}} _{q} ({\rm {\bf A}}^{
* }{\rm {\bf A}})_{.\,q} \left( {{\rm {\bf a}}_{.{\kern 1pt} p}^{
*} } \right))},
\end{equation}
\begin{equation}\label{kyr13}
\mid{\rm {\bf A}}\mid_{pq}= \frac{{\rm{ddet}}{ \rm{\bf
A}}\cdot\overline{{\rm{rdet}} _{p} ({\rm {\bf A}}{\rm {\bf A}}^{
* })_{p\,.} \left( {{\rm {\bf a}}_{q{\kern 1pt}. }^{
*} } \right)}}{{\rm n}({\rm{rdet}} _{p} ({\rm {\bf A}}{\rm {\bf
A}}^{* })_{p\,.} \left( {{\rm {\bf a}}_{q{\kern 1pt}.}^{ *} }
\right))}.
\end{equation}
\fi
\end{theorem}
\begin{proof}
Пусть ${\bf A}^{-1}=(b_{ij})$ - матрица
обратная матрице $\bf A$. Равенство
\EqRef{j i quasideterminant definition}
раскрывает связь между квазидетерминантом
$\mid\bfA\mid_{p,q}$ матрицы $\bfA \in {\rm M}(n,{\rm
{\mathbb{H}}})$ и элементами обратной матрицы $\bfA^{-1}=(b_{ij})$, а
именно
\[\mid\bfA\mid_{pq}=b_{qp}^{-1}\]
 для всех
$p$, $q=1$, ..., $n$. В тоже время теория строчных-столбцовых
определителей (теорема \ref{theorem: deter_inver}) дает нам
представления обратной матрицы через ее двойные левые \EqRef{left
inverse matrix} и правые \EqRef{right inverse matrix}
алгебраические дополнения. Таким образом, соответственно,
получим
\begin{equation}\label{kyr10}
  \mid\bfA\mid_{pq}=b_{qp}^{-1}=\left(\frac{{\mathbb{L}} _{pq}}{{\rm{ddet}}\bfA}\right)^{-1} =\left(\frac{{\rm{cdet}} _{q} (\bfA^{ * }{\rm
{\bf A}})_{.\,q} \left( {\bfA_{.{\kern 1pt} p}^* }
\right)}{{\rm{ddet}}\bfA}\right)^{-1},
\end{equation}
\begin{equation}\label{kyr11}
  \mid\bfA\mid_{pq}=b_{qp}^{-1}=\left(\frac{{\mathbb{R}} _{pq}}{{\rm{ddet}}\bfA}\right)^{-1} =\left(\frac{{\rm{rdet}} _{p} (\bfA{\rm
{\bf A}}^{ * })_{p\,.} \left( {\bfA_{q{\kern 1pt} .}^*
} \right)}{{\rm{ddet}}\bfA}\right)^{-1}.
\end{equation}
Так как ${\rm{ddet}}\bfA\neq 0\in {\rm {\mathbb{F}}}$,
то $\exists ({\rm{ddet}}\bfA)^{-1}\in {\rm
{\mathbb{F}}}$. В свою очередь
\begin{equation}\label{kyr14}
 {{\rm{cdet}} _{q} (\bfA^{
* }\bfA)_{.\,q} \left( {\bfA_{.{\kern 1pt} p}^{
*} } \right)}^{-1}=\frac{\overline{{\rm{cdet}} _{q} (\bfA^{
* }\bfA)_{.\,q} \left( {\bfA_{.{\kern 1pt} p}^{
*} } \right)}}{{\rm n}({\rm{cdet}} _{q} (\bfA^{
* }\bfA)_{.\,q} \left( {\bfA_{.{\kern 1pt} p}^{
*} } \right))},
\end{equation}
\begin{equation}\label{kyr15}
 {{\rm{rdet}} _{p} (\bfA\bfA^{
* })_{p\,.} \left( {\bfA_{q{\kern 1pt} .}^{
*} } \right)}^{-1}=\frac{\overline{{\rm{rdet}} _{p} ({\rm {\bf
A}}\bfA^{
* })_{p\,.} \left( {\bfA_{q{\kern 1pt}. }^{
*} } \right)}}{{\rm n}({\rm{rdet}} _{p} (\bfA{\rm {\bf
A}}^{* })_{p\,.} \left( {\bfA_{q{\kern 1pt}.}^* }
\right))}.
\end{equation}
Подставив (\ref{kyr14}) в (\ref{kyr10}), а (\ref{kyr15}) в
(\ref{kyr11}), соответственно получим (\ref{eq: quasi column determinant, 1}) и
(\ref{eq: quasi row determinant, 1}).

Теорема доказана.
\end{proof}

 Формула (\ref{eq: quasi column determinant, 1})
дает явное представление квазидетерминанта $\mid\bfA\mid_{p,q}$
матрицы $\bfA \in {\rm M}(n,{\rm {\mathbb{H}}})$ для всех
$p,q=1,...,n$ через  столбцовый определитель ее соответственной
левой эрмитовой матрицы ${\rm {\bf A}}^{* }\bfA$, а (\ref{eq: quasi row determinant, 1})
- через строчный определитель ее соответственной правой эрмитовой
${\rm {\bf A}}\bfA^{* }$.


\begin{example}
\label{example: quasideterminant, matrix 2x2}
%Пример 1.
Рассмотрим матрицу
\ShowEq{inverse matrix 2x2, 0}
Согласно \EqRef{quasideterminant, 1}
\ShowEq{quasideterminant, matrix 2x2}
Наша задача найти этот квазидетерминант, пользуясь теоремой
\ref{theorem: quasi row column determinant}.
Очевидно, что
\[\begin{array}{cc}
   \bfA^*=\begin{pmatrix}
   \BAA & \BAB \\
   \BBA & \BBB
 \end{pmatrix} & \bfA^*\bfA=\begin{pmatrix}
   {\rm n}(\AAA)+{\rm n}(\ABA) &
   \BAA\AAB+\BAB\ABB \\
   \BBA\AAA+\BBB\ABA
   & {\rm n}(\AAB)+{\rm n}(\ABB)
 \end{pmatrix}.
\end{array}
\]
Вычисляем необходимые определители
\[
\begin{array}{r@{\ }l}
  {\rm ddet}\bfA&={\rm rdet}_1(\bfA^*\bfA)\\
  &=({\rm n}(\AAA)+{\rm n}(\ABA))\cdot ({\rm n}(\AAB)+{\rm n}(\ABB))
\\
&-(\BAA\AAB+\BAB\ABB)\cdot
(\BBA\AAA+\BBB\ABA)  \\
  &={\rm n}(\AAA){\rm n}(\AAB)+{\rm n}(\AAA){\rm n}(\ABB)+{\rm
n}(\ABA){\rm n}(\AAB)+{\rm n}(\ABA){\rm n}(\ABB) \\
  &-\BAA\AAB\BBA\AAA-\BAA\AAB\BBB\ABA-
  \BAB\ABB\BBA\AAA-\BAB\ABB\BBB\ABA\\
&={\rm n}(\AAA){\rm n}(\ABB)+{\rm n}(\ABA){\rm
n}(\AAB)-(\BAA\AAB\BBB\ABA+\overline{\BAA\AAB\BBB\ABA})\\
&={\rm n}(\AAA){\rm n}(\ABB)+{\rm n}(\ABA){\rm n}(\AAB)-{\rm
t}(\BAA\AAB\BBB\ABA)
\end{array}
\]

\[
\begin{array}{r@{\ }l}
  {\rm cdet}_1(\bfA^*\bfA)_{.1}({\bf a}_{.2}^*)&=
  {\rm{cdet}}_1\begin{pmatrix}
    \BAB & \BAA\AAB+\BAB\ABB \\
    \BBB & {\rm n}(\AAB)+{\rm n}(\ABB)
  \end{pmatrix} \\
  &={\rm n}(\AAB) \BAB+ {\rm n}(\ABB) \BAB-\BAA\AAB\BBB-\BAB\ABB \BBB
\\
&={\rm n}(\AAB)
\BAB-\BAA\AAB\BBB.
  \end{array}
\]
Тогда,
\[
 \overline{{\rm{cdet}}_1(\bfA^*\bfA)_{.1}({\bf a}_{.2}^*)}={\rm
 n}(\AAB)\ABA-\ABB\BBA\AAA,
\]
\[\begin{array}{r@{\ }l}
  {\rm n}({\rm{cdet}}_1(\bfA^*\bfA)_{.1}({\bf a}_{.2}^*))&=
 \overline{{\rm{cdet}}_1(\bfA^*\bfA)_{.1}({\bf a}_{.2}^*)}\cdot{\rm{cdet}}_1(\bfA^*\bfA)_{.1}({\bf
 a}_{.2}^*) \\
 &= ({\rm
 n}(\AAB)\ABA-\ABB\BBA\AAA)\cdot({\rm n}(\AAB)
\BAB-\BAA\AAB\BBB) \\
&=  {\rm
 n}^{2}(\AAB){\rm
 n}(\ABA)-{\rm
 n}(\AAB)\ABA\BAA\AAB\BBB
 \\&-
{\rm
 n}(\AAB)\ABB\BBA\AAA\BAB+\ABB\BBA\AAA\BAA\AAB\BBB \\
&={\rm
 n}(\AAB)({\rm n}(\AAB){\rm n}(\ABA)-{\rm
t}(\BAA\AAB\BBB\ABA)+{\rm
n}(\ABA){\rm n}(\AAB))
\\
&={\rm
 n}(\AAB){\rm{ddet}}\bfA.
\end{array}
\]
Следуя формуле \eqref{eq: quasi column determinant, 1}, получим
\begin{equation}
\EqLabel{quasi column determinant, 2}
\begin{array}{r@{\ }l}
   |\bfA|_{21}&=\displaystyle
   \frac{{\rm{ddet}}\bfA
}{{\rm n}({\rm{cdet}}_1({\rm {\bf
A}}^*\bfA)_{.1}({\bf a}_{.2}^*))}
\overline{{\rm cdet}_1(\bfA^*\bfA)_{.1}({\bf a}_{.2}^*)}
\\&=\displaystyle
   \frac{{\rm ddet}\bfA }{{\rm
 n}(\AAB){\rm{ddet}}\bfA}
 \overline{{\rm{cdet}}_1(\bfA^*\bfA)_{.1}({\bf a}_{.2}^*)}
 \\&=\displaystyle
  \frac1{{\rm
 n}(\AAB)}\cdot\overline{{\rm{cdet}}_1(\bfA^*{\rm {\bf
A}})_{.1}({\bf a}_{.2}^*)}\\
&=\displaystyle\frac 1{{\rm
 n}(\AAB)}\cdot({\rm
 n}(\AAB)\ABA-\ABB\BBA\AAA)
 \\&=\ABA-\ABB(\AAB)^{-1}\AAA.
\end{array}
\end{equation}
Последнее выражение в \eqref{eq: quasi column determinant, 2}
совпадает с выражением $|{\rm
{\bf A}}|_{21}$ в \EqRef{quasideterminant, matrix 2x2}.
\qed
\end{example}


==> Rdtmt.Russian.tex <==
%auto-ignore
\input{Rdtmt.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Определитель по столбцам}
\fi

\section{Кватернионная алгебра}

%Какое обозначение Вам больше нравится?
%\ShowEq{Which notation is better}

\AddIndex{Кватернионная алгебра}{quaternion algebra}
\ShowEq{quaternion algebra H a b}
(она также обозначается как
\ShowEq{quaternion algebra F a b}
)
- это четырехмерное векторное пространство над полем ${\rm
{\mathbb{F}}}$ 
с базисом $\{1,i,j,k\}$ и следующими
правилами умножения:
\[\begin{array}{c}
  i^{2}=a, \\
  j^{2}=b, \\
  ij=k, \\
  ji=-k.
\end{array}
\]
Поле ${\rm
{\mathbb{F}}}$ является центром кватернионной алгебры
${\rm {\mathbb{H}}}( a,b)$.

В алгебре ${\rm {\mathbb{H}}}( a,b)$ определены следующие отображения.
\begin{itemize}
\item
Квадратичная форма
\ShowEq{norm, quaternion algebra}
такая что
\ShowEq{norm 1, quaternion algebra}
называется 
\AddIndex{нормой}{norm, quaternion algebra}
в кватернионной алгебре ${\mathbb{H}}$.
\item
Линейное отображение
\ShowEq{trace, quaternion algebra}
называется
\AddIndex{следом кватерниона}{trace, quaternion algebra}.
След удовлетворяет
\AddIndex{условию перестановочности следа}{permutability property of trace}
\ShowEq{permutability property of trace}
Из теоремы
\xRef{0701.238}{theorem: Quaternion over real field, matrix}
следует
\ShowEq{trace 3, quaternion algebra}
\item
Линейное отображение
\ShowEq{involution, quaternion algebra}
является
\AddIndex{инволюцией}{involution, quaternion algebra}.
Инволюция имеет следующие свойства
\ShowEq{involution 1, quaternion algebra}
При этом кватернион
\ShowEq{involution 2, quaternion algebra}
будем называть
\AddIndex{сопряженным к кватерниону}{conjugate of quaternion} 
$x\in {\rm {\mathbb{H}}}$.
Норма и инволюция удовлетворяют следующему условию
\ShowEq{norm 2, quaternion algebra}
След и инволюция удовлетворяют следующему условию
\ShowEq{trace 2, quaternion algebra}
Из равенств
\EqRef{trace 3, quaternion algebra},
\EqRef{involution, quaternion algebra}
следует
\ShowEq{involution 3, quaternion algebra}
\end{itemize}

В зависимости от выбора поля ${\rm {\mathbb{F}}}$ и
элементов $ a, b$     на множестве всех кватернионных
алгебр  возможны два случая
\citeBib{Lewis D. W. Quaternion algebras}:

1.$\Fab F$ является алгеброй с
делением.

2. $\Fab F$ изоморфна алгебре
всех $2\times 2$ матриц над полем ${\rm {\mathbb{F}}}$. В этом
случае кватернионная алгебра - расщепляемая.

Рассмотрим некоторые  не изоморфные кватернионные алгебры с
делением.

1. $\Fab R$, где ${\rm
{\mathbb{R}}}$ - поле действительных чисел, изоморфна
классическому телу кватернионов ${\bf H}$, когда $a<0$  и
$b<0$.  В противном случае, $\Fab R$ - расщепляемая.

2. Над полем рациональных чисел ${\rm {\mathbb{Q}}}$ существует
бесконечно много не изоморфных кватернионных алгебр с делением
$\Fab Q$ в зависимости от
выбора $a<0$  и $b<0$.

3. Пусть ${\rm {\mathbb{Q}}}_{p}$  - поле $p$-адичних чисел, где
$p$ - простое число. Для каждого простого числа $p$ существует
единственная кватернионная алгебра с делением.

\section{Введение в теорию строчных и столбцовых определителей}
\label{section: row column determinant}

Строчные и столбцовые определители вводятся для матриц над
кватернионной алгеброй ${\rm {\mathbb{H}}}$.
Следующие определения в теории подстановок необходимы нам для
введения строчно-столбцовых определителей.

\begin{definition} Пусть
\ShowEq{symmetric group}
-- симметрическая группа на множестве $I_n = \{1,2,...,n\}$
(\citeBib{Serge Lang}, с. 70, упражнения 9, 10). Будем говорить, что
подстановка $\sigma \in S_n $ образует прямое произведение
независимых циклов, если ее запись в обычной двухрядной форме
соответствует ее разложению в независимые циклы
\begin{equation}\label{kyr2}
\sigma =
\begin{pmatrix}
  n_{11} & n_{12} & \ldots & n_{1l_1} & \ldots & n_{r1} & n_{r2} & \ldots & n_{rl_{r}}\\
  n_{12} & n_{13} & \ldots & n_{11} & \ldots & n_{r2} & n_{r3} & \ldots & n_{r1}
\end{pmatrix}
\end{equation}
\qed
\end{definition}

\begin{definition}
Будем говорить, что представление \eqref{kyr2} подстановки
$\sigma$ произведением независимых циклов является
\AddIndex{упорядоченным слева}{left-ordered cycle notation of permutation},
если элементы, которые замыкают каждый из ее
  независимых циклов, записываются первыми слева в каждом из циклов
\[
\sigma = \left( {n_{11} n_{12} \ldots n_{1l_1} } \right)\,\left(
{n_{21} n_{22} \ldots n_{2l_{2}} }  \right)\ldots \left( {n_{r1}
n_{r2} \ldots n_{rl_{r}} }  \right).
\]
\qed
\end{definition}

\begin{definition}
Будем говорить, что представление \eqref{kyr2} подстановки
$\sigma$ произведением независимых циклов является
\AddIndex{упорядоченным справа}
{right-ordered cycle notation of permutation},
если элементы, которые замыкают каждый из ее независимых
циклов, записываются первыми справа в каждом из циклов
\[
\sigma = \left(  n_{12} \ldots n_{1l_1}{n_{11} } \right)\,\left(
 n_{22} \ldots n_{2l_{2}}{n_{21} }  \right)\ldots \left(
n_{r2} \ldots n_{rl_{r}} {n_{r1}}  \right).
\]
\qed
\end{definition}

\begin{definition}
Пусть $S_n $ -- симметрическая группа на множестве $I_n=\{1,2,...,n\}$.
Пусть $ i \in \overline {1,n}$.
\AddIndex{Строчным определителем}{row determinant} по  $i$-й
строке матрицы $\bfA=(a_{ij}) \in {\rm M}\left( {n,{\rm
{\mathbb{H}}}} \right)$ будем
называть выражение
\ShowEq{row determinant}
Это выражение является альтернированной суммой  $n!$ мономов,
составленных из элементов матрицы  ${\rm {\bf A}}$,
в каждом из
которых подстановка $\sigma \in S_n $ индексов образует прямое
произведение независимых циклов
\ShowEq{row determinant permutation}
%И если подстановка четная, то
%моном берется со знаком "плюс", а если нечетная,  то -- "минус".
В упорядоченном слева разложении  подстановки  $\sigma $
первый слева цикл начинается слева индексом $i$, а все
следующие циклы удовлетворяют условиям:
 \[
 i_{k_{2}}  < i_{k_{3}}  < \ldots < i_{k_{r}}  {\rm ,}
\quad i_{k_{t}}  < i_{k_{t} + s} {\rm ,} \quad \left( {\forall t =
\overline {2,r}}  \right){\rm ,} \quad \left( {\forall s =
\overline {1,l_{t}} }  \right).
\]
\qed
\end{definition}

\begin{definition}
Пусть  $S_n $  -- симметрическая группа на множестве $J_n =\{1,2,...,n\}$.
Пусть $ j \in \overline {1,n}$.
\AddIndex{Столбцовым определителем}{column determinant}
по $j$-му столбцу  матрицы $\bfA=(a_{ij}) \in {\rm M}\left( {n,{\rm
{\mathbb{H}}}} \right)$ будем называть выражение
\ShowEq{column determinant}
Это выражение является альтернированной суммой $n!$ мономов,
составленных из элементов матрицы  ${\rm {\bf A}}$,
в каждом из которых подстановка $\tau \in S_n $ индексов
образует прямое произведение независимых циклов
\ShowEq{column determinant permutation}
%И если подстановка четная, то
%моном берется со знаком "плюс", а если нечетная,  то -- "минус".
В упорядоченном справа разложении подстановки  $\tau $
первый справа цикл
начинается справа индексом $j$, а все следующие циклы
удовлетворяют условиям:
\[ j_{k_{2}}  < j_{k_{3}}  < \ldots < j_{k_{r}},
\quad j_{k_{t}}  < j_{k_{t} + s}, \quad \left( {\forall t =
\overline {2,r}}  \right), \quad \left( {\forall s = \overline
{1,l_{t}} }  \right).
\]
\qed
\end{definition}

\begin{remark}
Особенностью столбцовых определителей является то, что при
непосредственном их вычислении  множители каждого из мономов
записываются справа налево.
\qed
\end{remark}

В леммах \ref{lemma: right decomposition of determinant} и
\ref{lemma: left decomposition of determinant} рассмотрено
рекуррентное определение столбцовых и строчных определителей. Это
определение является аналогом разложения определителя по строкам и
столбцам в коммутативном случае.

\begin{lemma}
\label{lemma: right decomposition of determinant}%kyrc1}
Пусть
\ShowEq{right cofactor, matrix}
-- \AddIndex{правое алгебраическое дополнение}{right cofactor, matrix}
 элемента  $a_{i{\kern 1pt} j} $ матрицы
$\bfA=(a_{ij}) \in {\rm M}\left( {n,{\rm {\mathbb{H}}}}
\right)$, а именно
\ShowEq{right cofactor 1, matrix}
Тогда
\ShowEq{right decomposition of determinant}
где матрица $\Aci$
получается
из $\bfA$ последовательным применением замены   $j$-го
столбца $i$-м и вычеркивания $i$-х строки и столбца.
\qed
\end{lemma}

\begin{lemma}
\label{lemma: left decomposition of determinant}
Пусть
\ShowEq{left cofactor, matrix}
-- \AddIndex{левое алгебраическое дополнение}{left cofactor, matrix}
элемента $a_{i{\kern 1pt} j}$ матрицы
$\bfA=(a_{ij}) \in {\rm M}\left( {n,{\rm {\mathbb{H}}}} \right)$, а именно
\ShowEq{left cofactor 1, matrix}
Тогда
\ShowEq{left decomposition of determinant}
где матрица $\Arj$
получается из  $\bfA$
последовательным применением замены   $i$-й строки $j$-й и
вычеркивания $j$-х строки и столбца.
\qed
\end{lemma}

\begin{remark}
Очевидно, что каждому моному любого определенного выше
детерминанта квадратной матрицы отвечает моном любого другого
детерминанта, строчного или столбцового, такой, что оба они имеют
одинаковый знак,
 состоят из одних и тех же множителей, - элементов матрицы, и отличаются
  только порядком их размещения.
Кроме того, если элементы матрицы коммутируют, то $ {\rm{rdet}}
_1\, \bfA = \ldots = {\rm{rdet}} _{{n}} \bfA =
{\rm{cdet}}_1\, \bfA = \ldots = {\rm{cdet}} _{{n}}
\bfA. $
\qed
\end{remark}

Рассмотрим основные свойства строчного и столбцового детерминанта
  произвольной квадратной матрицы над телом ${\rm {\mathbb{H}}}$, доказательства
   которых непосредственно следуют из определений.

\begin{theorem}
Если одна из строк (столбцов) матрицы  $\bfA\in {\rm
M}\left( {n,{\rm {\mathbb{H}}}} \right)$  состоит из нолей, тогда
для всех $i = \overline {1,n}$
\[{\rm{rdet}}_{{i}}\, \bfA
= 0, \quad  {\rm{cdet}} _{{i}}\, \bfA = 0. \]
\end{theorem}

\begin{theorem}
Если $i$-я строка  матрицы  $\bfA=(a_{ij})\in {\rm M}\left(
{n,{\rm {\mathbb{H}}}} \right)$ умножается слева на любое $b \in
{\rm {\mathbb{H}}} $, тогда для всех $i = \overline {1,n}$
\[ {\rm{rdet}}_{{i}}\,\rowcolAc{i{\kern 1pt}.}{b\cdot\colA i} = b \cdot
{\rm{rdet}}_{{i}}\, \bfA.\]
\end{theorem}

\begin{theorem}
Если $j$-й столбец матрицы
$\bfA=(a_{ij})\in {\rm M}\left( {n,{\rm {\mathbb{H}}}}
\right)$ умножается справа на  любое $b \in {\rm {\mathbb{H}}}$,
тогда для всех $j = \overline {1,n}$
\[{\rm{cdet}} _j\,\rowcolAc{.{\kern 1pt}j}{\rowA j\cdot b}  = {\rm{cdet}}
_j\, \bfA \cdot b.\]
\end{theorem}

\begin{theorem}
Если для $\bfA=(a_{ij})\in {\rm M}\left(
{n,{\rm {\mathbb{H}}}} \right)$ найдется такое $ k \in I_n $,
что $a_{kj} = b_{j} + c_{j} $ для всех $j = \overline {1,n}$,
тогда для любого $i = \overline {1,n}$
\[
\begin{array}{c}
   {\rm{rdet}}_{{i}}\, \bfA = {\rm{rdet}}_{{i}}\, {\rm {\bf
A}}_{{k{\kern 1pt}.}} \left( {{\rm {\bf b}}} \right) +
{\rm{rdet}}_{{i}}\, \bfA_{{k{\kern 1pt}.}} \left( {{\rm
{\bf c}}} \right), \\
  {\rm{cdet}} _{{i}}\, \bfA = {\rm{cdet}} _{{i}}\, {\rm
{\bf A}}_{{k{\kern 1pt}.}} \left( {{\rm {\bf b}}} \right) +
{\rm{cdet}}_{{i}}\, \bfA_{{k{\kern 1pt}.}} \left( {{\rm
{\bf c}}} \right).
\end{array}
\]
где ${\rm {\bf b}}=(b_1,\ldots, b_n)$, ${\rm {\bf
c}}=(c_1,\ldots, c_n).$
\end{theorem}

\begin{theorem}
Если для $\bfA=(a_{ij})\in {\rm M}\left(
{n,{\rm {\mathbb{H}}}} \right)$ найдется такое $ k \in I_n $,
что $a_{i\,k} = b_{i} + c_{i} $ для всех $ i = \overline {1,n}$,
тогда для любого $j = \overline {1,n}$
\[
\begin{array}{c}
  {\rm{rdet}}_j\, \bfA = {\rm{rdet}}_j\, {\rm {\bf
A}}_{{.\,k}} \left( {{\rm {\bf b}}} \right) + {\rm{rdet}}_j\,
\bfA_{{.\, k}} \left( {{\rm {\bf c}}} \right),\\
  {\rm{cdet}} _j\, \bfA = {\rm{cdet}} _j\, {\rm
{\bf A}}_{{.\,k}} \left( {{\rm {\bf b}}} \right) + {\rm{cdet}}
_j \bfA_{{.\,k}} \left( {{\rm {\bf c}}} \right).
\end{array}
\]
где ${\rm {\bf b}}=(b_1,\ldots, b_n)^{T}$, ${\rm {\bf
c}}=(c_1,\ldots, c_n)^{T}.$
\end{theorem}

\begin{theorem}
Пусть $\bfA^* $
-- матрица, эрмитово сопряженная к  $\bfA\in {\rm M}\left( {n,{\rm
{\mathbb{H}}}} \right)$, тогда $ {\rm{rdet}}_{{i}}\, {\rm {\bf
A}}^* =\overline{{\rm{cdet}} _{{i}}\, \bfA}$ для
любого $i = \overline {1,n}. $
\qed
\end{theorem}

Следующая теорема имеет ключевое значение в теории строчных и
столбцовых определителей.

\begin{theorem}
\label{theorem: determinant of hermitian matrix}
Если $\bfA=(a_{ij}) \in {\rm M}\left( {n,{\rm {\mathbb{H}}}}
\right)$ -- эрмитовая матрица, тогда
\[
{\rm{rdet}}_1 \bfA = \ldots = {\rm{rdet}} _n \bfA
= {\rm{cdet}}_1 \bfA = \ldots = {\rm cdet}_n
\bfA  \in {\rm {\mathbb{F}}}.
\]
\qed
\end{theorem}

\begin{remark}
\label{remark: determinant of hermitian matrix}
Поскольку все столбцовые и строчные определители
 эрмитовой матрицы над телом ${\rm {\mathbb{H}}}$ равны между собой,
 то мы можем однозначно ввести понятие определителя
 эрмитовой матрицы ${\rm {\bf A}}\in
{\rm M}\left( {n,{\rm {\mathbb{H}}}} \right)$:
 \ShowEq{determinant of hermitian matrix}
\qed
\end{remark}

\begin{remark}
Представляя детерминант эрмитовой матрицы как строчный
 определитель по произвольной $i$-й строке по лемме
 \ref{lemma: right decomposition of determinant} имеем
\ShowEq{right decomposition of hermetean determinant}
Сравнивая выражения
\EqRef{determinant, recursive definition, kyr}
и
\eqref{eq: right decomposition of hermetean determinant}
для эрмитовой
матрицы $\bfA \in {\rm M}\left( {n,\bf{H}} \right)$, с
очевидностью получаем, что введенный строчный определитель для
эрмитовой матрицы совпадает с детерминантом Мура, а строчные и
столбцовые определители для произвольных матриц являются его
обобщением на множестве произвольных квадратных матриц.
\qed
\end{remark}

Свойства определителя эрмитовой матрицы полностью рассматриваются
в \citeBib{0702447} посредством ее строчных и столбцовых определителей.
Среди всех рассмотрим следующие.

\begin{theorem}
Если $i$-ю строку эрмитовой матрицы $\bfA\in {\rm
M}\left( {n,{\rm {\mathbb{H}}}} \right)$
 заменить левой линейной комбинацией  других ее строк
\ShowEq{substitute row i by linear combination}
 где $ c_{l} \in {\rm {\mathbb{H}}}$ для всех $l =
\overline {1,k}$ и $\{i,i_{l}\}\subset I_n $, 
тогда для всех
$i=\overline{1,n}$
\ShowEq{substitute row i by linear combination, determinant}
\qed
\end{theorem}

\begin{theorem}
Если  $j$-й столбец эрмитовой матрицы
 $\bfA\in {\rm
M}\left( {n,{\rm {\mathbb{H}}}} \right)$ заменить правой
линейной
  комбинацией  других ее столбцов
\ShowEq{substitute col j by linear combination}
где $c_{l} \in {\rm {\mathbb{H}}}$ для всех $l = \overline {1,k}$ и
$\{j,j_{l}\}\subset J_n$ , тогда для всех $j=\overline{1,n}$
\ShowEq{substitute col j by linear combination, determinant}
\qed
\end{theorem}

Следующая теорема о детерминантном представлении матрицы обратной
к эрмитовой непосредственно следует из этих свойств.

\begin{theorem}
\label{theorem: unique right and left inverse Hermitian matrix}
Для эрмитовой невырожденной матрицы
$\bfA \in {\rm M}\left( {n,{\rm {\mathbb{H}}}} \right)$,
( $\det \bfA \ne 0$), существует единственная правая
 $(R\bfA)^{ - 1}$ и единственная левая
обратная матрица $(L\bfA)^{ - 1}$, при этом $\left(
{R\bfA} \right)^{ - 1} = \left( {L\bfA}
\right)^{ - 1} = :\bfA^{ - 1}$, которые обладают
следующими детерминантными представлениями:
\ShowEq{unique right and left inverse Hermitian matrix}
Здесь $R_{ij}$,  $L_{ij}$ являются соответственно левым и правым
алгебраическими дополнениями для всех $i,j = \overline {1,n}$.
\qed
\end{theorem}

Для того, чтобы получить детерминантное представление для
произвольной обратной матрицы над телом ${\rm {\mathbb{H}}}$
рассматриваются ее правая $\bfA\bfA^* $ и
левая $\bfA^*\bfA $ соответственные эрмитовые
матрицы.

\begin{theorem}[\citeBib{0702447}]
\label{theorem: column rank of matrix}
Если произвольный столбец матрицы $\bfA\in {\rm {\mathbb{H}}}^{m\times n} $ является
правой линейной комбинацией ее других столбцов, или произвольная
строка матрицы $\bfA^*$ является
левой линейной комбинацией ее других строк, тогда $\det \bfA^* \bfA = 0.$
\qed
\end{theorem}

Поскольку главная подматрица эрмитовой матрицы эрмитова, то
главный базисный минор может быть определен  по аналогии с
коммутативным случаем, как ненулевой определитель ее главной
подматрицы максимального порядка. Также вводим понятие
\AddIndex{ранга эрмитовой матрицы по главным минорам}
{rank of Hermitian matrix by principal minors},
 как максимальный порядок отличного от
нуля главного минора. Следующая теорема
устанавливает соответствие между ним и рангом матрицы определенным
как максимальное количество  линейно независимых столбцов справа
или  линейно независимых строк слева, которые и образуют базис.

\begin{theorem}[\citeBib{0702447}]
\label{theorem: rankA} 
Ранг по главным минорам эрмитовой матрицы $\bfA^* {\rm
{\bf A}}$ равняется ее рангу, а также рангу матрицы $\bfA
\in {\rm {\mathbb{H}}}^{m\times n}$.
\qed
\end{theorem}

\begin{theorem}[\citeBib{0702447}]
Если $\bfA \in {\rm {\mathbb{H}}}^{m\times n}$, тогда
произвольный столбец матрицы  $\bfA$ является правой
линейной комбинацией ее базисных столбцов или произвольная
строка матрицы $\bfA$ является левой линейной комбинацией
ее базисных строк.
\qed
\end{theorem}

Отсюда следует критерий вырожденности соответственной эрмитовой
матрицы.

\begin{theorem}[\citeBib{0702447}]
\label{theorem: ddetA=0}
Правая линейная независимость столбцов матрицы $\bfA \in
{\rm {\mathbb{H}}}^{m\times n}$ или левая линейная независимость
строк матрицы  $\bfA^* $ является необходимым и
достаточным условием того, что
\ShowEq{ddetA=0}
\end{theorem}

\begin{theorem}[\citeBib{0702447}]
\label{theorem: determinant A A star = A star A}
Если $\bfA \in {\rm M}\left( {n,{\rm {\mathbb{H}}}}
\right)$, тогда $\det \bfA\bfA^* = \det \bfA^* \bfA$.
\qed
\end{theorem}

\begin{example}
Рассмотрим матрицу
\[
\bfA=
\begin{pmatrix}
\AAA&\AAB
\\
\ABA&\ABB
\end{pmatrix}
\]
Тогда
\[
\bfA^*=
\begin{pmatrix}
\BAA&\BAB
\\
\BBA&\BBB
\end{pmatrix}
\]
Соответственно
\[
\bfA\bfA^*=
\begin{pmatrix}
\AAA\BAA+\AAB\BBA
&
\AAA\BAB+\AAB\BBB
\\
\ABA\BAA+\ABB\BBA
&
\ABA\BAB+\ABB\BBB
\end{pmatrix}
\]
\[
\bfA^*\bfA=
\begin{pmatrix}
\BAA\AAA+\BAB\ABA
&
\BAA\AAB+\BAB\ABB
\\
\BBA\AAA+\BBB\ABA
&
\BBA\AAB+\BBB\ABB
\end{pmatrix}
\]
Чтобы оценить детерминанты полученных эрмитовых матриц,
рассмотрим например первый строчный
определитель каждой матрицы.
Согласно теореме \ref{theorem: determinant of hermitian matrix}
и замечанию \ref{remark: determinant of hermitian matrix}
\begin{align*}
\det\bfA\bfA^*&={\rm rdet}_1 \bfA\bfA^*
\\
\det\bfA^*\bfA&={\rm rdet}_1 \bfA^*\bfA
\end{align*}
Согласно лемме \ref{lemma: right decomposition of determinant}
\begin{align}
\EqLabel{row 1 determinant A A star}
\begin{array}{r@{\ }l}
\det\bfA\bfA^*&=
(\bfA\bfA^*)_{11}(\bfA\bfA^*)_{22}-(\bfA\bfA^*)_{12}(\bfA\bfA^*)_{21}
\\
&=(\AAA\BAA+\AAB\BBA)(\ABA\BAB+\ABB\BBB)
\\
&-(\AAA\BAB+\AAB\BBB)(\ABA\BAA+\ABB\BBA)
\\
&=\AAA\BAA\ABA\BAB+\AAB\BBA\ABA\BAB
\\
&+\AAA\BAA\ABB\BBB+\AAB\BBA\ABB\BBB
\\
&-\AAA\BAB\ABA\BAA-\AAB\BBB\ABA\BAA
\\
&-\AAA\BAB\ABB\BBA-\AAB\BBB\ABB\BBA
\\
&=\AAB\BBA\ABA\BAB+\AAA\BAA\ABB\BBB
\\
&-\AAB\BBB\ABA\BAA-\AAA\BAB\ABB\BBA
\end{array}
\\
\EqLabel{row 1 determinant A star A}
\begin{array}{r@{\ }l}
\det\bfA^*\bfA&=
(\bfA^*\bfA)_{11}(\bfA^*\bfA)_{22}-(\bfA^*\bfA)_{12}(\bfA^*\bfA)_{21}
\\
&=(\BAA\AAA+\BAB\ABA)(\BBA\AAB+\BBB\ABB)
\\
&-(\BAA\AAB+\BAB\ABB)(\BBA\AAA+\BBB\ABA)
\\
&=\BAA\AAA\BBA\AAB+\BAB\ABA\BBA\AAB
\\
&+\BAA\AAA\BBB\ABB+\BAB\ABA\BBB\ABB
\\
&-\BAA\AAB\BBA\AAA-\BAB\ABB\BBA\AAA
\\
&-\BAA\AAB\BBB\ABA-\BAB\ABB\BBB\ABA
\\
&=\BAB\ABA\BBA\AAB+\BAA\AAA\BBB\ABB
\\
&-\BAB\ABB\BBA\AAA-\BAA\AAB\BBB\ABA
\end{array}
\end{align}
Положительные слагаемые в равенствах \eqref{eq: row 1 determinant
A A star}, \eqref{eq: row 1 determinant A star A} являются
действительными числами и, очевидно, совпадают. Чтобы доказать
равенство
\begin{equation}\label{kyr16}
a_{12}\overline{a_{22}}a_{21}\overline{a_{11}}+a_{11}\overline{a_{21}}a_{22}\overline{a_{12}}
=\overline{a_{21}}a_{22}\overline{a_{12}}a_{11}+\overline{a_{11}}a_{12}\overline{a_{22}}a_{21}
\end{equation}
используем свойство перестановочности следа элементов
кватернионной алгебры, ${\rm t}(pq)={\rm t}(qp)$. Действительно,
\[a_{12}\overline{a_{22}}a_{21}\overline{a_{11}}+a_{11}\overline{a_{21}}a_{22}\overline{a_{12}}=
a_{12}\overline{a_{22}}a_{21}\overline{a_{11}}+\overline{a_{12}\overline{a_{22}}a_{21}\overline{a_{11}}}=
{\rm t}(a_{12}\overline{a_{22}}a_{21}\overline{a_{11}}),\]
\[\overline{a_{21}}a_{22}\overline{a_{12}}a_{11}+\overline{a_{11}}a_{12}\overline{a_{22}}a_{21}=
\overline{\overline{a_{11}}a_{12}\overline{a_{22}}a_{21}}+\overline{a_{11}}a_{12}\overline{a_{22}}a_{21}={\rm
t}(\overline{a_{11}}a_{12}\overline{a_{22}}a_{21})\] Тогда из
свойства перестановочности следа, следует (\ref{kyr16}).
\qed
\end{example}

\def\theDate{15 September}
\ifx\KyrcheiComment\theDate Однако равенство
\begin{equation}
\EqLabel{2 row determinants}
\AAB\BBB\ABA\BAA+\AAA\BAB\ABB\BBA
=
\BAB\ABB\BBA\AAA+\BAA\AAB\BBB\ABA
\end{equation}
не столь очевидно.

Равенство \eqref{eq: 2 row determinants} является следствием следующей теоремы.

\begin{theorem}
Равенство
\begin{equation}
\EqLabel{sum transposition conjugation}
a_1...a_n+\overline{a_n}...\overline{a_1}=
\sigma(a_1)...\sigma(a_n)+\overline{\sigma(a_n)}...\overline{\sigma(a_1)}
\end{equation}
верно для любых кватернионов $a_1$, ..., $a_n$ и
любой перестановки
\[
\sigma=
\begin{pmatrix}
a_1&...&a_n
\\
\sigma(a_1)&...&\sigma(a_n)
\end{pmatrix}
\]
\end{theorem}
%\begin{proof}
Мы можем переписать равенство
\eqref{eq: sum transposition conjugation}
в виде равенства
\begin{equation}
\EqLabel{sum transposition conjugation, 1}
a_1...a_n+\overline{a_1...a_n}=
\sigma(a_1)...\sigma(a_n)+\overline{\sigma(a_1)...\sigma(a_n)}
\end{equation}
после чего становится очевидным, что с обеих сторон равенства у нас стоит действительное выражение.
Пусть
\begin{align*}
a&=a_0+a_1i+a_2j+a_3k
\\
b&=b_0+b_1i+b_2j+b_3k
\end{align*}
Тогда
\[
Re(ab)=a_0b_0-a_1b_1-a_2b_2-a_3b_3
\]
Индукцией по числу множителей нетрудно убедиться, что выражение
\[
a_1...a_n+\overline{a_1...a_n}
\]
симметрично по переменным $a_1$, ..., $a_n$. Это утверждение завершает доказательство
равенства
\eqref{eq: sum transposition conjugation}.

\def\theDate{August 19}
\ifx\AleksComment\theDate
Мы докажем утверждение индукцией по $n$.

Если $n=2$, то
\[
\sigma=
\begin{pmatrix}
a_1&a_2
\\
a_2&a_1
\end{pmatrix}
\]
единственная нетривиальная перестановка,
и равенство \eqref{eq: sum transposition conjugation}
имеет вид
\begin{equation}
\EqLabel{sum transposition conjugation, n=2}
a_1a_2+\overline a_2\overline a_1
=
a_2a_1+\overline a_1\overline a_2
\end{equation}
Поскольку сумма в правой и левой частях равенства
\eqref{eq: sum transposition conjugation, n=2} является действительным
числом, то для доказательства равенства
\eqref{eq: sum transposition conjugation, n=2} достаточно
записать выражение для действительной компоненты произведения
%Равенство \eqref{eq: sum transposition conjugation, n=2} верно, так как
%$a_1a_2+\overline a_2\overline a_1$ - действительная величина, и кроме того,
%правая часть есть выражение, сопряжённое левой части.

Пусть равенство \eqref{eq: sum transposition conjugation}
справедливо для $k=n-1$. Рассмотрим произвольную перестановку
\[
\sigma=
\begin{pmatrix}
a_1&...&a_n
\\
\sigma(a_1)&...&\sigma(a_n)
\end{pmatrix}
\]

%a+a*=b+b*=>ca+a*c* v cb+b*c*
%abcd+d*c*b*a*=bcda+a*d*c*b*
abcdf+f*d*c*b*a*=adcbf+f*b*c*d*a*
|
V
bcdfa*^{-1}+a^{-1}f*d*c*b*=dcbfa*^{-1}+a^{-1}f*b*c*d*
fa*^{-1}->f,a^{-1}f*=>f*
|
V
bcdf+f*d*c*b*=dcbf+f*b*c*d*
=>bcdf=cbdf=cdbf=dcbf?
bcdf=cdfb=fbcd=bcdf

Если $\sigma(a_n)=a_n$, то перестановка
Выберем такие $i$, $j$, что $\sigma(a_i)=a_n$, $\sigma(a_n)=a_j$.
Тогда
\begin{align*}
\sigma&=\sigma_1\circ\sigma_2
\\
\sigma_1&=
\begin{pmatrix}
a_1&...&a_i&...&a_j&...&a_n
\\
\sigma(a_1)&...&a_j&...&a_i&...&\sigma(a_n)
\end{pmatrix}
\\
\sigma_2&=
\begin{pmatrix}
a_1&...&a_i&...&a_j&...&a_n
\\
a_1&...&a_n&...&a_i&...&a_j
\end{pmatrix}
\end{align*}
\fi
%\end{proof}

Равенство \eqref{eq: 2 row determinants}
следует из равенства
\eqref{eq: sum transposition conjugation},
если положить $n=4$, $a_1= \AAB$, $a_2=\BBB$, $a_3=\ABA$, $a_4=\BAA$
и выбрать перестановку
\[
\sigma=
\begin{pmatrix}
\AAB&\BBB&\ABA&\BAA
\\
\BAA&\AAB&\BBB&\ABA
\end{pmatrix}
\]

%Самое интересное здесь – это то что неравенство нетривиально. Хотя складываются числа равные по модулю, но их направление может быть разным и это не гарантирует равенство проекций на действительную ось. Интересно и другое. Обе величины отсутствуют в любом из двойных определителей. Поэтому напрашивается обобщение, что
%не зависит от перестановки s. Но я рассмотрел только определители второго порядка. Возможно это равенство справедливо для любого чётного(?) набора множителей. Я думаю что оно уже где-то доказано
\fi

 На основании теоремы \ref{theorem: determinant A A star = A
star A} вводится понятие двойного определителя. Впервые это
понятие было введено Л. Ченом (\citeBib{L. Chen: Definition of determinant}).

\begin{definition}
Определитель эрмитовой матрицы $\bfA\bfA^*$ называется
\AddIndex{двойным определителем}{double determinant} матрицы $\bfA
\in {\rm M}\left( {n,{\rm {\mathbb{H}}}} \right)$
\ShowEq{double determinant}
\qed
\end{definition}

В случае если ${\rm {\mathbb{H}}}$ - классическое тело
кватернионов ${\bf H}$ над полем действительных чисел, тогда
имеет место теорема, которая устанавливает справедливость
Аксиомы 1 для двойного определителя.

\begin{theorem}
Если ${\left\{
{\bfA,{\rm {\bf B}}} \right\}} \subset {\rm M}\left( {n,{\rm {\bf
H}}} \right)$, тогда ${\rm{ddet}} \left( {{\rm {\bf A}} \cdot {\rm
{\bf B}}} \right) = {\rm{ddet}}\bfA \cdot{\rm{ddet}} {\rm {\bf
B}}.$
\qed
\end{theorem}

В общем случае не существует взаимосвязей между
вырожденностью двойного определителя матрицы и её строчными и
столбцовыми определителями. Продемонстрируем это в следующем
примере.

\begin{example}
 Рассмотрим матрицу $$A=\begin{pmatrix}
  i & j \\
  j  & -i
\end{pmatrix}$$
Ее вторая строка получена из первой умножением слева на $k$. Тогда
согласно теореме \ref{theorem: ddetA=0} ${\rm{ddet}} A=0$.
Действительно,
\[A^{*}A=\begin{pmatrix}
  -i & -j \\
  -j  & i
\end{pmatrix}\cdot \begin{pmatrix}
  i & j \\
  j  & -i
\end{pmatrix}=\begin{pmatrix}
  2 & -2k \\
  2k  & 2
\end{pmatrix}. \]
Тогда ${\rm{ddet}} A= 4+4k^2=0$, но $${\rm{cdet}}_1 A={\rm{cdet}}_2
A={\rm{rdet}}_1 A={\rm{rdet}}_2 A=-i^2-j^2=2$$ B то же время
$rankA=1$, что соответствует теореме \ref{theorem: rankA}.
\qed
\end{example}

Установлено соответствие между двойным определителем и
некоммутативными определителями Мура, Стади и Дьедонне,
\[{\rm ddet} \bfA = {\rm Mdet} \left( {\bfA^*
\bfA} \right) = {\rm Sdet} \bfA = {\rm Ddet}
^{2}\bfA\]

\begin{definition}
Пусть
\ShowEq{left double cofactor}
тогда будем называть
\ShowEq{left double cofactor 1}
\AddIndex{левым двойным алгебраическим дополнением}{left double cofactor}
элемента $a_{ij}$ матрицы $\bfA \in {\rm M}\left(
{n,{\rm {\mathbb{H}}}} \right)$.
\qed
\end{definition}

\begin{definition}
Пусть
\ShowEq{right double cofactor}
тогда будем называть
\ShowEq{right double cofactor 1}
\AddIndex{правым двойным алгебраическим дополнением}{right double cofactor}
элемента $a_{ij} $ матрицы $\bfA \in {\rm
M}\left( {n,{\bf H}} \right)$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: deter_inver}
Необходимым и достаточным условием обратимости
матрицы $\bfA=(a_{ij}) \in {\rm M}(n,{\rm {\mathbb{H}}})$
является ${\rm{ddet}} \bfA \ne 0$. Тогда $\exists {\rm
{\bf A}}^{ - 1} = \left( {L\bfA} \right)^{ - 1} = \left(
{R\bfA} \right)^{ - 1}$, где
\begin{equation}
\EqLabel{left inverse matrix}
\left( {L\bfA} \right)^{ - 1} =\left( {{\rm
{\bf A}}^*\bfA } \right)^{ - 1}\bfA^*
={\frac{1}{{{\rm{ddet}}\bfA }}}
\begin{pmatrix}
  {\mathbb{L}} _{11} & {\mathbb{L}} _{21}& \ldots & {\mathbb{L}} _{n1} \\
  {\mathbb{L}} _{12} & {\mathbb{L}} _{22} & \ldots & {\mathbb{L}} _{n2} \\
  \ldots & \ldots & \ldots & \ldots \\
 {\mathbb{L}} _{1n} & {\mathbb{L}} _{2n} & \ldots & {\mathbb{L}} _{nn}
\end{pmatrix}
\end{equation}
\begin{equation}
\EqLabel{right inverse matrix}
\left( {R\bfA} \right)^{ - 1} = {\rm {\bf
A}}^* \left( {\bfA\bfA^* } \right)^{ - 1}
= {\frac{1}{{{\rm{ddet}}\bfA^* }}}
\begin{pmatrix}
 {\mathbb{R}} _{\,{\kern 1pt} 11} & {\mathbb{R}} _{\,{\kern 1pt} 21} &\ldots & {\mathbb{R}} _{\,{\kern 1pt} n1} \\
 {\mathbb{R}} _{\,{\kern 1pt} 12} & {\mathbb{R}} _{\,{\kern 1pt} 22} &\ldots & {\mathbb{R}} _{\,{\kern 1pt} n2}  \\
 \ldots  & \ldots & \ldots & \ldots \\
 {\mathbb{R}} _{\,{\kern 1pt} 1n} & {\mathbb{R}} _{\,{\kern 1pt} 2n} &\ldots & {\mathbb{R}} _{\,{\kern 1pt} nn}
\end{pmatrix}
\end{equation}
и ${\mathbb{L}} _{ij} = {\rm{cdet}} _{j} (\bfA^{ * }{\rm
{\bf A}})_{.\,j} \left( {\bfA_{.{\kern 1pt} i}^* }
\right)$, ${\mathbb{R}} _{\,{\kern 1pt} ij} = {\rm{rdet}}_{i}
(\bfA\bfA^*) _{i.} \left( {{\rm {\bf
A}}_{j\,.}^* }  \right), \left( {\forall i,j = \overline {1,n}}
\right)$.
\qed
\end{theorem}

\begin{corollary}
Пусть ${\rm{ddet}} \bfA \ne 0$. Тогда
\[
\mathbb{L}_{ij}=\mathbb{R}_{ij}
\]
\qed
\end{corollary}

\begin{remark}
Теорема \ref{theorem: deter_inver} представляет обратную матрицу $\bfA^{ - 1}$
произвольной квадратной матрицы $\bfA \in {\rm M}(n,{\rm
{\mathbb{H}}})$, если ${\rm{ddet}}\bfA \ne 0$, через
аналог классической присоединенной. Если мы обозначим ее ${\rm
Adj}{\left[ {{\left[ {\bfA} \right]}} \right]}$, тогда
над телом  ${\rm {\mathbb{H}}}$ имеет место следующая формула:
\[
\bfA^{ - 1} = {\frac{{{\rm Adj}{\left[ {{\left[ {{\rm
{\bf A}}} \right]}} \right]}}}{{{\rm{ddet}} \bfA}}}.
\]
\qed
\end{remark}

Очевидным следствием детерминантного представления обратной
матрицы через аналог классической присоединенной матрицы
является правило Крамера.

\begin{theorem}
\label{theorem: right_system}
Пусть
\ShowEq{right_system}
правая система линейных уравнений  с матрицей коэффициентов
$\bfA \in {\rm M}(n,{\rm {\mathbb H}})$, столбцом свободных
элементов ${\rm {\bf y}} = \left( {y_1 ,\ldots ,y_n }
\right)^{T}\in {\rm {\mathbb{H}}}^{n\times 1}$ и столбцом
неизвестных ${\rm {\bf x}} = \left( {x_1 ,\ldots ,x_n}
\right)^{T}$. Если ${\rm{ddet}}\bfA \ne 0$, тогда система
линейных уравнений
\EqRef{right_system} имеет единственное решение, которое представляется
формулой:
\ShowEq{Cramer_rule_right_syst}
где  ${\rm {\bf f}} = \bfA^* {\rm {\bf y}}.$
\qed
\end{theorem}

\begin{theorem}
Пусть
\ShowEq{left_syst}
-- левая система линейных уравнений  с матрицей коэффициентов
$\bfA \in {\rm M}(n,{\rm {\mathbb{H}}})$, строкой свободных
элементов ${\rm {\bf y}} = \left( {y_1 ,\ldots ,y_n } \right)\in
{\rm {\mathbb{H}}}^{1\times n}$ и строкой неизвестных
${\rm {\bf x}} = \left( {x_1 ,\ldots ,x_n} \right)$. Если ${\rm{ddet}}{
\rm{\bf A}} \ne 0$, тогда система
линейных уравнений \EqRef{left_syst} имеет единственное
решение, которое представляется формулой:
\ShowEq{Cramer_rule_left_syst}
где $ {\rm {\bf z}} = {\rm {\bf y}}\bfA^* .$
\qed
\end{theorem}

Формулы
\EqRef{Cramer_rule_right_syst}
и \EqRef{Cramer_rule_left_syst} являются
естественным и очевидным обобщением правила Крамера для квадратных
систем линейных уравнений над кватернионной алгеброй с делением.
Еще более близкую аналогию
 можно получить в следующих частных случаях, которые следуют из
 теоремы \ref{theorem: unique right and left inverse Hermitian matrix}.

\begin{theorem}
Пусть в правой системе линейных уравнений \EqRef{right_system}
 матрица коэффициентов $\bfA \in {\rm
M}(n,{\rm {\mathbb{H}}})$ -- эрмитова. Тогда система имеет
единственное решение, которое представляется формулой:
\[
x_{j} = {\frac{{{\rm{cdet}} _{j} \bfA_{.j} \left( {{\rm
{\bf y}}} \right)}}{{\det \bfA}}}, \quad \left( {\forall
j = \overline {1,n}}  \right).
\]
\qed
\end{theorem}

\begin{theorem}
Пусть в левой системе линейных уравнений
  \EqRef{left_syst} матрица коэффициентов $\bfA \in {\rm M}(n,{\rm {\mathbb{H}}})$
  -- эрмитова. Тогда система имеет единственное решение, которое
представляется формулой:
\[
x_{i}^{} = {\frac{{{\rm{rdet}}_{i} \bfA_{i.} \left( {{\rm
{\bf y}}} \right)}}{{\det \bfA}}}, \quad \left( {\forall
i = \overline {1,n}}  \right).
\]
\qed
\end{theorem}

В рамках теории строчных-столбцовых определителей получено также
правило Крамера для правого $\bfA{\rm {\bf X}} = {\rm
{\bf B}}$, левого ${\rm {\bf X}}\bfA = {\rm {\bf B}}$ и
двустороннего $\bfA{\rm {\bf X}}{\rm {\bf B}} = {\rm {\bf
C}}$ матричных уравнений (\citeBib{1004.4380}). Также получено детерминантное
представление Мура\Hyph Пенроуза обратной матрицы над телом кватернионов и
правило Крамера для нормального решения правой и левой систем
линейных уравнений (\citeBib{1005.0736}).


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%A%0
\Symb%
   {$(^a_b)$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb%
   {минор}%
   {A from b a}%
\Symb%
   {минор}%
   {A from columns T}%
\Symb%
   {минор}%
   {A from rows S}%
\Symb%
   {минор}%
   {A without column a}%
\Symb%
   {минор}%
   {A without columns T}%
\Symb%
   {минор}%
   {A without row b}%
\Symb%
   {минор}%
   {A without rows S}%
\Symb%
   {активное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%
   {активное представление группы $G(\Vector  f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {active representation in basis manifold, tower of representations}%
\Symb%
   {аффинное пространство}%
   {affine space, division ring}%
\Symb%
   {аффинное пространство}%
   {An}%
\Symb%
   {ассоциатор $R$\Hyph алгебры}%
   {associator of algebra}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb%
   {коммутатор $R$\Hyph алгебры}%
   {commutator of algebra}%
\Symb%
   {компонента линейного отображения $\Vector{A}$ $D$\Hyph векторного пространства}%
   {component of linear map, D vector space}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {CR linear combination in A module}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb%
   {\drc вектор}%
   {drc vector}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
\Symb%
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb%
   {частное линейное отображение переменной $v^i$}%
   {partial linear map of variable}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
\Symb%
   {множество $A$\Hyph линейных отображений модуля $\Vector V$ в модуль $\Vector W$}%
   {set A linear maps, module}%
\Symb%
   {множество линейных отображений тела $D_1$ в тело $D_2$}%
   {set linear maps, division ring}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Symb%
   {правый сдвиг}%
   {starT shift}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {левый сдвиг}%
   {Tstar shift}%
\Symb%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Symb%
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%

\SetIndexSpace%C%0
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Symb%
   {структурные константы алгебры $A$ над кольцом $D$}%
   {structural constants of algebra}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
\Symb%
   {координаты базового вектора представления группы Ли}%
   {basis vector of representation of Lie group, coordinates}%
\Symb%
   {компонента производной Гато отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of map, algebra}%
\Symb%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Symb%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of Second Order, algebra}%
\Symb%
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$ тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Symb%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$ алгебры}%
   {Gateaux derivative of map, algebra}%
\Symb%
   {производная Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Symb%
   {производная Гато отображения $f$ алгебры}%
   {Gateaux derivative of map, fraction, algebra}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, algebra}%
\Symb%
   {производная Гато второго порядка отображения $\Vector f$}%
   {Gateaux derivative of Second Order, D vector space}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, division ring}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%
   {дифференциал Гато отображения $f$ алгебры}%
   {Gateaux differential of map, algebra}%
\Symb%
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Symb%
   {дифференциал Гато второго порядка отображения $f$ алгебры}%
   {Gateaux differential of Second Order, algebra}%
\Symb%
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Symb%
   {дифференциал Гато второго порядка отображения $f$ тела}%
   {Gateaux differential of Second Order, division ring}%
\Symb%
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 1, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 2, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 3, D vector space}%
\Symb%
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Symb%
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 1, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 2, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 3, D vector space}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb%
   {производная Картана}%
   {overbrace D}%
\Symb%
   {производная}%
   {overline D}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb%
   {\drc векторное пространство \subs строк}%
   {r rows drc vector space}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
\Symb%
   {стандартная компонента производной Гато отображения $f$}%
   {standard component of Gateaux derivative, algebra}%
\Symb%
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Symb%
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Symb%
   {тензорное произведение колец}%
   {tensor product of rings}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%
   {$A\CRcirc$\Hyph базис модуля}%
   {A CRcirc basis, module over algebra}%
\Symb%
   {аффинный базис}%
   {Affine Basis}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
\Symb%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
\Symb%
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%
   {координаты базиса в \rcd векторном пространстве \sups строк}%
   {basis coordinates, c rows rcd vector space}%
\Symb%
   {координаты базиса в \drc векторном пространстве \subs строк}%
   {basis coordinates, r rows drc vector space}%
\Symb%
   {базис в \rcd векторного пространства \sups строк}%
   {basis, c rows rcd vector space}%
\Symb%
   {базис в \drc векторном пространстве \subs строк}%
   {basis, r rows drc vector space}%
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb%
   {компонента полилинейного отображения ассоциативной алгебры}%
   {component of polylinear map, associative algebra}%
\Symb%
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb%
   {норма отображения в $D$\Hyph алгебру}%
   {norm of map, algebra}%
\Symb%
   {норма отображения $f$  тела}%
   {norm of map, division ring}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of Tstar representation of group}%
\Symb%
   {ортонормальный базис}%
   {Orthonornal Basis, division ring}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
\Symb%
   {система отсчёта}%
   {reference frame}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb%
   {стандартная $F$\Hyph компонента линейного отображения $f$ }%
   {standard component of linear map, division ring}%
\Symb%
   {стандартная компонента полилинейного отображения в ассоциативную алгебру}%
   {standard component of polylinear map, associative algebra}%
\Symb%
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb%
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb%
   {алгебра Ли группы Ли}%
   {g}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
\Symb%
   {малая группа элемента $x$}%
   {little group}%
\Symb%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective covariant starT representation of group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective covariant Tstar representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective covariant Tstar representation of group}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, 1 n}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
\Symb%
   {алгебра кватернионов над полем действительных чисел}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%
   {ядро линейного отображения $D$\Hyph векторного пространства}%
   {kernel of linear map, D vector space}%
\Symb%
   {ядро линейного отображения тела}%
   {kernel of linear map, division ring}%

\SetIndexSpace%L%0
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%
   {предел последовательности в нормированном кольце}%
   {limit of sequence, normed ring}%
\Symb%
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
\Symb%
   {множество \Acr линейных отображений модуля $\Vector V$ в модуль $\Vector W$}%
   {set Acr linear maps, module}%
\Symb%
   {\rcd векторное пространство \drc линейных отображений \drc векторного пространства $\Vector V$ в \drc векторное пространство $\Vector W$}%
   {set drc linear maps, drc vector space}%
\Symb%
   {множество линейных отображений алгебры $A_1$ в алгебру $A_2$}%
   {set linear mappings, algebra}%
\Symb%
   {множество линейных отображений $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector{W}$}%
   {set linear maps, D vector space}%
\Symb%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%
\Symb%
   {множество $n$\hyph линейных отображений алгебры $A$ в модуль $S$}%
   {set polylinear mappings An, algebra}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$  в модуль $S$}%
   {set polylinear mappings, algebra}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
\Symb%
   {\drc векторное пространство \rcd линейных отображений \rcd векторного пространства $\Vector{V}$ в \rcd векторное пространство $\Vector{W}$}%
   {set rcd linear maps, rcd vector space}%
\Symb%
   {множество \sT представлений тела $S$ в аддитивной группе тела $R$}%
   {set sT representations, division ring}%
\Symb%
   {множество \Ts представлений тела $S$ в аддитивной группе тела $R$}%
   {set Ts representations, division ring}%

\SetIndexSpace%M%0
\Symb%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb%
   {множество преобразований множества $M$}%
   {set of transformations}%
\Symb%
   {множество \Ts преобразований универсальной алгебры $M$}%
   {set of Tstar transformations}%
\Symb%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
\Symb%
   {ядро $R$\Hyph алгебры $A$}%
   {nucleus of algebra}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb%
   {пассивное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {passive representation in basis manifold}%
\Symb%
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {passive representation in basis manifold, tower of representations}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
\Symb%
   {\rcd векторное пространство \sups строк}%
   {c rows rcd vector space}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
\Symb%
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
\Symb%
   {правый сдвиг}%
   {right shift}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
\Symb%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%
\Symb%
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Symb%
   {образ базиса $X$ при пассивном преобразовании $S$}%
   {passive transformation of basis, representation}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%

\SetIndexSpace%T%0
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Symb%
   {касательная плоскость к группе $G$}%
   {TaG}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%

\SetIndexSpace%V%0
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Symb%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb%
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Symb%
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Symb%
   {векторное пространство}%
   {V}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to generating set, representation}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Symb%
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
\Symb%
   {суперпозиция координат эндоморфизма представления $f$ и точки $m$}%
   {superposition of coordinates, representation}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
\Symb%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%
   {центр $R$\Hyph алгебры $A$}%
   {center of algebra}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
\Symb%
   {связность}%
   {conection overline}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%

\SetIndexSpace%Fi%2
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
\Symb%
   {произведение групп $G_i$, $i\in I$}%
   {product of groups}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, i 1 n}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb%
   {подрасслоение}%
   {subbundle}%

\CloseIndex

